A pragmatic workflow for research software engineering in computational science

University research groups in Computational Science and Engineering (CSE) generally lack dedicated funding and personnel for Research Software Engineering (RSE), which, combined with the pressure to maximize the number of scientific publications, shifts the focus away from sustainable research software development and reproducible results. The neglect of RSE in CSE at University research groups negatively impacts the scientific output: research data - including research software - related to a CSE publication cannot be found, reproduced, or re-used, different ideas are not combined easily into new ideas, and published methods must very often be re-implemented to be investigated further. This slows down CSE research significantly, resulting in considerable losses in time and, consequentially, public funding. We propose a RSE workflow for Computational Science and Engineering (CSE) that addresses these challenges, that improves the quality of research output in CSE. Our workflow applies established software engineering practices adapted for CSE: software testing, result visualization, and periodical cross-linking of software with reports/publications and data, timed by milestones in the scientific publication process. The workflow introduces minimal work overhead, crucial for university research groups, and delivers modular and tested software linked to publications whose results can easily be reproduced. We define research software quality from a perspective of a pragmatic researcher: the ability to quickly find the publication, data, and software related to a published research idea, quickly reproduce results, understand or re-use a CSE method, and finally extend the method with new research ideas.

==> ieee-preamble.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%             IEEE PREAMBLE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \documentclass[format=sigconf]{acmart}
% % \documentclass{llncs}

% \settopmatter{printacmref=false} % Removes citation information below abstract
% \renewcommand\footnotetextcopyrightpermission[1]{} % removes footnote with conference information in first column
% \pagestyle{plain} % removes running headers

%% The amssymb package provides various useful mathematical symbols
%\usepackage{amssymb}

% \author{Tomislav Mari\'{c}}
% \affiliation{\department{Mathematics Department}\institution{TU Darmstadt}\city{Darmstadt}\country{Germany}}
% \email{maric@mma.tu-darmstadt.de}

% \author{Dennis Gläser}
% \affiliation{\department{Mathematics Department}\institution{TU Darmstadt}\city{Darmstadt}\country{Germany}}
% \email{maric@mma.tu-darmstadt.de}

% \author{Jan-Patrick Lehr}
% \affiliation{\department{Computer Science}\institution{TU Darmstadt}\city{Darmstadt}\country{Germany}}
% \email{jan-patrick.lehr@tu-darmstadt.de}

% \author{Ioannis Papagiannidis}
% \affiliation{\department{Mathematics Department}\institution{TU Darmstadt}\city{Darmstadt}\country{Germany}}


% \author{Benjamin Lambie}
% \affiliation{\department{Thermo-Fluids \& Interfaces}\institution{TU Darmstadt}\city{Darmstadt}\country{Germany}}
% \email{lambie@tfi.tu-darmstadt.de}

% \author{Christian Bischof}
% \affiliation{\department{Computer Science}\institution{TU Darmstadt}\city{Darmstadt}\country{Germany}}
% \email{christian.bischof@tu-darmstadt.de}

% \author{Dieter Bothe}
% \affiliation{\department{Mathematics Department}\institution{TU Darmstadt}\city{Darmstadt}\country{Germany}}
% \email{bothe@mma.tu-darmstadt.de}

%\renewcommand{\sectionname}{Section}
% \acmYear{2021}
%\acmConference[PASC'21]{PASC}{July, 05 -- 08}{Geneva, Switzerland}

% \keywords{research software engineering, research data management, data science, research workflow}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%            END IEEE PREAMBLE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> ms.tex <==
% \input{ieee-preamble}

\input{elsevier-preamble}

\input{packages}


\newcommand{\dg}[1]{\color{black}#1\color{black}\xspace}
\newcommand{\jp}[1]{\color{black}#1\color{black}}
\newcommand{\tm}[1]{\textcolor{black}{#1}}
\newcommand{\eg}{e.g.\@\xspace}

\title{A Research Software Engineering Workflow for Computational Science and Engineering}

\begin{document}


\input{sections/abstract}

\maketitle

%%% TODO: Remove for submission
\thispagestyle{plain}
\pagestyle{plain}


% \section{Venue Info}
% Current idea is to target PASC.
% \begin{itemize}
%     \item Full paper: 13th December 2020
%     \item Format: ACM
%     \item Pages: 10 including all (figs, tables, references)
%     \item Abstract: 200 words
%     \item \url{https://pasc21.pasc-conference.org/submission/guidelines-for-papers/}
%     \item PASC, Geneva (or virtual)
%     \item double blind review
% \end{itemize}


%% main text

\linenumbers
\input{sections/introduction.tex}
\input{sections/scientific-software-quality-workflow.tex}
\input{sections/minimal-working-example.tex}
\input{sections/case-studies}
\input{sections/conclusions.tex}


\section*{Acknowledgements}
This work was funded by the Deutsche Forschungsgemeinschaft (DFG, German Research Foundation) -- Project-ID 265191195 -- SFB 1194, and by the Hessian LOEWE initiative within the Software-Factory 4.0 project.
The authors would also like to thank the Federal Government and the Heads of Government of the Länder, as well as the Joint Science
Conference (GWK), for their funding and support within the framework of the NFDI4Ing consortium. Funded by the German Research
Foundation (DFG) - project number 442146713.
Benchmarks were conducted on the Lichtenberg cluster at TU Darmstadt.

The authors are grateful to Moritz Schwarzmeier for his work on the NFDI4Ing Knowledgebase \citep{NFDI4IngKBase}, and to Moritz Schwarzmeier and Tobias Tolle for providing valuable constructive feedback on the RSE workflow and this manuscript.

%% The Appendices part is started with the command \appendix;
%% appendix sections are then done as normal sections
%% \appendix

%% \section{}
%% \label{}

% IEEE bibliography
% \bibliographystyle{IEEEtran}
%\bibliography{IEEEabrv,literature.bib}

% Elsevier bibliography
\bibliographystyle{elsarticle-num-names} 
\bibliography{literature.bib}

%% End of file `elsarticle-template-num-names.tex'.

\end{document}


==> packages.tex <==
%% The amssymb package provides various useful mathematical symbols
%\usepackage{amssymb}
%\usepackage{textcomp}
%\usepackage{mathtools}
%\usepackage{subcaption}
%\usepackage[section]{placeins}
%% The amsthm package provides extended theorem environments
%% \usepackage{amsthm}

%% The lineno packages adds line numbers. Start line numbering with
%% \begin{linenumbers}, end it with \end{linenumbers}. Or switch it on
%% for the whole article with \linenumbers.
%\usepackage{lineno}

%% standardize citation format
%\usepackage[numbers]{natbib}
%\usepackage{listings}
%\renewcommand{\lstlistingname}{Code}% Listing -> Algorithm
%\renewcommand{\lstlistlistingname}{List of \lstlistingname s}% List of Listings -> List of Algorithms

%\usepackage{hyperref}
%\usepackage{float}
%\usepackage{algorithm}
%\usepackage{graphicx}
%\usepackage{algpseudocode}
%\usepackage{amsmath}
%\usepackage[size=footnotesize]{subcaption}
%\usepackage[textsize=tiny,disable]{todonotes}
%\graphicspath{{figures/}}
%\usepackage{cleveref}
%\usepackage{soul}
%\usepackage{geometry}
%\floatsetup[listing]{style=Plaintop}
%\setlength{\marginparwidth}{2cm}
%\usepackage{algorithmicx}
%\usepackage{booktabs}
%\usepackage{longtable}
%\usepackage{stmaryrd}
%\usepackage[inline]{enumitem}
%\usepackage{xspace}

%\usepackage[utf8]{inputenc}

%\usepackage{comment}
%%\includecomment{CiSE}
%\excludecomment{CiSE}


%\newenvironment{enuminline}{\begin{enumerate*}[label=(\arabic*)]}{\end{enumerate*}}
%\newenvironment{enumi}{\begin{enumerate*}[label=(\arabic*)]}{\end{enumerate*}}
%\newenvironment{enumialph}{\begin{enumerate*}[label=(\alph*)]}{\end{enumerate*}}

%\newcommand{\cl}{\emph{C}}
%\newcommand{\cppl}{\cl\texttt{++}}
%\newcommand{\minwf}{minimum workflow}
%\newcommand{\Minwf}{Minimum workflow}
%\newcommand{\fuwf}{full workflow}
%\newcommand{\Fuwf}{Full workflow}


==> sections/abstract.tex <==
\begin{abstract}


University research groups in Computational Science and Engineering (CSE) generally lack dedicated funding and personnel for Research Software Engineering (RSE), which, combined with the pressure to maximize the number of scientific publications, shifts the focus away from sustainable research software development and reproducible results. The neglect of RSE in CSE at University research groups negatively impacts the scientific output: research data - including research software - related to a CSE publication cannot be found, reproduced, or re-used, different ideas are not combined easily into new ideas, and published methods must very often be re-implemented to be investigated further. This slows down CSE research significantly, resulting in considerable losses in time and, consequentially, public funding.


We propose a RSE workflow for Computational Science and Engineering (CSE) that addresses these challenges, that improves the quality of research output in CSE. Our workflow applies established software engineering practices adapted for CSE: software testing, result visualization, and periodical cross-linking of software with reports/publications and data, timed by milestones in the scientific publication process. The workflow introduces minimal work overhead, crucial for university research groups, and delivers modular and tested software linked to publications whose results can easily be reproduced. We define research software quality from a perspective of a pragmatic researcher: the ability to quickly find the publication, data, and software related to a published research idea, quickly reproduce results, understand or re-use a CSE method, and finally extend the method with new research ideas.

% A workflow for increasing research software quality is proposed, based on cross-linking scientific publications, software, and data, while ensuring the reproducibility of results.
% The focus is placed on research software in Computational Science and Engineering (CSE), and the proposed workflow addresses in a straightforward way several challenges in increasing and maintaining research software quality in CSE.
% Specifically, CSE software is usually complex and large-scale, which complicates the organization of feature contributions and tests.
% Furthermore, testing CSE software requires High-Performance Computing (HPC) resources.
% The proposed workflow addresses these and other challenges by applying best practices from Software Development and adapting them to the requirements in CSE.
\end{abstract}


% German abstract

==> sections/build-system-short.tex <==
\subsection{Build system}
\label{ssec:build-system}

\todo[inline]{PASC review: This sec on remains very abstract and vague.}

Adoption of open source software and the complexity of scientific codes often introduce a relatively large number of dependencies.
Using an established build system simplifies handling of dependencies on different platforms.
Rules can be defined in the build system that enable the same source code to be built on different systems, where the dependencies used by the scientific code are placed in different paths.
Moreover, build systems handle platform-dependent technical details and hence, reduce the time required to maintain the build process.
We strongly advocate the use of build systems instead of writing and maintaining platform-specific build instructions as e.g. GNU Makefiles. 

==> sections/build-system.tex <==
\subsection{Build system}
\label{ssec:build-system}

\todo[inline]{PASC review: This sec on remains very abstract and vague.}

Adoption of open source software and the complexity of scientific codes often introduce a relatively large number of dependencies.
Using an established build system simplifies handling of dependencies on different platforms.
Rules can be defined in the build system that enable the same source code to be built on different systems, where the dependencies used by the scientific code are placed in different paths.
Moreover, build systems handle platform-dependent technical details and hence, reduce the time required to maintain the build process.
We strongly advocate the use of build systems instead of writing and maintaining platform-specific build instructions as e.g. GNU Makefiles. 

==> sections/case-studies-short.tex <==
\section{Case studies}\label{sec:case-studies}

\todo[inline]{PASC review: results are not presented in a quantifiable manner (?) - the reader is left to trust the authors. Perhaps this is solved by a template repository.}

This section presents two software projects that follow the minimum workflow and apply, in addition, parts or all of the full workflow.
We highlight which parts of the workflow were introduced at what time of the project and how it helped to improve the software or its development process.

\input{sections/geophase-short.tex}

\input{sections/pira-short.tex}


==> sections/case-studies.tex <==
\section{Case studies}\label{sec:case-studies}

\todo[inline]{PASC review: results are not presented in a quantifiable manner (?) - the reader is left to trust the authors. Perhaps this is solved by a template repository.}

This section presents two software projects that follow the minimum workflow and apply, in addition, parts or all of the full workflow.
We highlight which parts of the workflow were introduced at what time of the project and how it helped to improve the software or its development process.

\input{sections/geophase.tex}

\input{sections/pira.tex}


==> sections/conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

The proposed Research Software Engineering workflow for Computational Science and Engineering significantly increases the quality of scientific results with a minimal workload overhead, which makes it applicable in a university research setting with limited dedicated resources for RSE. 
Placing the focus of the workflow on scientific publications makes the workflow attractive for researchers that already mainly develop CSE research software to generate scientific publications as their primary scientific output.

\dg{
The minimal workflow combines an established build system with a simple feature-based version-control branching model adapted to the peer-review process.
Submission, revision and acceptance of scientific publications are the main milestones
in this branching model, using git-tags and cross-links between data, software, and publications. This} ensures that the FAIR principles \citep{FAIR} are applied to a large extent in a challenging university research setting with an extremely low work overhead. 

The complete workflow further increases the sustainability of research software. Next to the known practice of issue tracking, our version of Test-Driven Development - adapted to CSE research software - gradually increases the test coverage of research software, allowing researchers to keep the focus on the subsequent scientific publication without introducing broad unit-testing unrelated to the research roadmap.
Automatic test quantification and result visualization using Jupyter notebooks in a data-processing pipeline provide a basis for discussions and data analysis that help in quickly identifying sources of errors.
Automatic testing combined with containerization and minimal workflow makes it possible to reproduce research results from any milestone across different computing platforms. 
Finally, the use of Continuous Integration for automating scientific workflows enables the results to be reproduced automatically from a git Web interface.
Granted, for researchers unfamiliar with the tools and techniques from the complete workflow, a non-negligible learning investment is expected.
However, this investment has a very high return rate. 
Increasing testing coverage using our version of TDD as well as automatic test quantification and visualization quickly pay off even for individual researchers and very small research groups. 
Continuous Integration increases research output more gradually once the time comes to combine existing research into new ideas. 




% The proposed workflow for increasing the quality of scientific software in its minimal form does not cause a significant workload overhead and it completely solves the following often encountered issues in Computational Science / Engineering: 
% \begin{enumi}
% \item not being able to find the data from a publication to compare it with new results,
% \item not being able to quickly understand which methodology is implemented by the scientific software,
% \item  not being able to re-use a model from one publication in another publication,
% \item  not being able to easily start a new development from a previous state,
% \item  not being able to derive new models based on existing results from a specific publication, and
% \item  not knowing who was responsible for a specific change in the source code.
% \end{enumi}

% The advanced version of the workflow incurs an overhead at the beginning of each project. 
% However, the benefits strongly outweigh this initial effort, because
% \begin{enumi}
% \item new additions to the team have an overview of the project in the issue tracking system and can start contributing more quickly and easily, 
% \item the Continuous Integration automates the quality check of a new feature that must otherwise be done manually by the researcher and costs a lot more time over the years than to configure it, 
% \item the containerization (specifically with Singularity) makes it possible to share not only result data, but also software, across heterogeneous platforms and without the effort of building the software on those platforms, 
% \item a handful of Test Driven Development practices outlined here are simple to learn and significantly increase software quality. 
% \end{enumi}


==> sections/containerization.tex <==
\subsection{Containerization}
\label{ssec:containerization}

\todo[inline]{PASC review: - It could be worth to men on that also the container les can be cross-linked}

The reproducibility of results is a fundamental principle of research.
% Reproducing results from scientific codes is not only relevant when one decides to derive new models based on an existing implementation / data. 
In addition, being able to use software in a productive environment is highly relevant. 
% The next logical question is then: Which environment?
However, the multitude of platforms provides a challenge, given the usually limited number of personnel in academic research groups, especially when required on top of the demanded FAIR principles~\citep{FAIR}.
% With limited resources it is not realistic to require from a research team (in Computational Engineering) to develop a cross-platform software, on top of requirements set by FAIR principles \citep{FAIR}.
An approach for cross-platform interoperability is the encapsulation of the software environment in so-called containers.
Containers, e.g., Singularity containers~\citep{Singularity, Kurtzer2017}, make it possible to execute software in any environment, given that it provides a suitable container runtime.
Hence, results can be reproduced more easily if the researcher provides containers that include the software and configuration files used for a specific publication. Large input data sets should not be included in the
container but should be published separately in a data repository. This keeps
the container size as small as possible, for instance, for users that want to
use the software on their own data set. For the reproduction of results, the
input data can be downloaded on-the-fly from the data repository.
% EDIT Dennis: changed "input data" to "configuration files" and added sentence
% \todo[inline]{@Dennis: I think I would be careful with "input data". I guess here it is referred to config files, etc, but not some large input files - which I think should be drawn from a related data repository instead of bloating the container. Maybe we can use "configuration files" or similar instead of input data?}

How the container is built is specified in \emph{recipe} files.
They list all required dependencies, the software, how it is built and which data to copy into the container. However, note that copying data into the
container makes the recipe itself not comply with the FAIR
principles~\citep{FAIR} as one cannot reproduce the building process without
that data. Therefore, it is beneficial to only use data from online
resources with a guarantee of availability, for instance, from dedicated data
repositories. The same holds also for code: one should prefer to pull used sources
from release pages or "git clone" into a repository with a specific commit or tag
in the build recipe instead of copying source code into the container. In general,
git repositories have no guarantee to exist over long time periods, as they could
in principle be moved or removed. Therefore, if available, one can clone into the
mirrors hosted at \href{https://www.softwareheritage.org/}{softwareheritage.org/}
which are guaranteed to be conserved over a long time frame.
% EDIT DENNIS: Added a sentence
% \todo[inline]{@Dennis: I personally would always try to NOT copy any data into a container, but try to make the recipe itself FAIR, that is, only use online available resources (from package manager, git clone available repos, etc.).}

Finally, the recipe could define a set of commands that can be invoked on the container, e.g., to reproduce a specific result.

% A container software with great potential in CSE is Singularity \citep{Singularity,Kurtzer2017}.
% Singularity is developed with an HPC focus and can therefore safely run on university clusters. 
% This is extremely useful for researchers, as it is no longer required to install dependencies or download additional software just to make another person's scientific software work.
% In fact, results can be reproduced with Singularity on any machine that supports it with a single command.

% There is some work overhead involved for the researcher, as  Singularity requires \textit{Definition files} to be written for the software.
% Definition files are  recipes for the construction of containers. 
% They define all the dependencies and input data data that should be be present in a container.
% However, this overhead is reasonable, as the result is the ability to run the executable applications and re-run their tests anywhere.


==> sections/continuous-integration.tex <==
\subsection{Continuous integration of research software}
\label{ssec:continuous-integration}

\begin{figure*}[!ht]
    \centering
    % \def\svgwidth{0.95\textwidth}
    % \footnotesize
    % \input{images/ZINF-CI-diagram-drawio.pdf_tex}
    \includegraphics[scale=0.5]{images/ZINF-CI-diagram.drawio.pdf}
    \caption{Continuous integration workflow: the merge request triggers the CI pipeline to execute. This builds the software, runs all tests and produces the visualizations. These are published for inspection. If tests pass, the merge request is accepted and the changes are added to the main repository. If the tests fail, the developer inspects the results and re-initiates the process.}
    \label{fig:ci_cd}
\end{figure*}

Continuous Integration~(CI)~\citep{Fowler2006} is the practice of frequent integration of changes in a shared version of the software.
% The goal of the increased frequency of integration is to prevent the situation where different features diverge strongly from each other, up to the point where it is very difficult to integrate them.
% This is unfortunately often the case for scientific codes developed at universities.
% Software design, re-integration and maintainability are all too often second-class citizens compared to features that can be presented in a publication.
% This causes developments that serve short-term, i.e., $1-4$ years long, projects done by a PostDoc / Ph.D. student and a few graduate students.
% Unfortunately, their developments are often never re-integrated into the main version of the scientific software.
% Repetition, TM.
In this section, a straightforward CI workflow is presented for research software, that increases its quality without introducing a significant workload overhead for the researchers.

To understand CI, and its benefits, it is beneficial to briefly reiterate the connected branching model, \emph{cf.}~\cref{ssec:vcs}.
A new feature is developed using a so-called \emph{feature branch} (research idea), while the current stable version of the software is maintained on the \emph{main branch}.
In a more traditional sense, CI recommends frequent, e.g., daily, integration from features onto the main branch.
Daily integration of changes is not tractable for scientific software, because the features are driven by scientific research: it is often not immediately clear if the developed methodology will work.
Therefore, this integration is performed when the generated results are suitable for the submission of a scientific publication to a peer-review process.
On the other hand, bug fixes and potential improvements to the main branch can be integrated into the feature branch.
% In the meantime, bug fixes or developments that are obviously valid (e.g. improve shared components), are done on the main branch.
% In the feature->main direction, the integration is not therefore not continuous, in fact, it is sporadic.
To anticipate diverging individual feature branches, this integration should be done frequently, e.g., weekly.
% However, since the scientific software is mostly developed further by multiple "individual" (Ph.D.) projects, one must ensure that they do not all diverge completely.
% Therefore, the integration direction main-to-feature should be done fairly often, say, at least weekly.
This ensures that improvements to common, shared components are integrated into the individual feature branches.
Moreover, integrating from main to feature branch on a weekly basis, makes sure that the developments achieved in a successful project are integrated by everyone in the research group, while the responsible developer is still working in the research group.
Hence, no working software artifact is lost.
% \paragraph{Embedding in workflow}

Even though the integration itself may not always be continuous, there are aspects of CI that help to increase code quality.
\cref{fig:ci_cd} shows a CI workflow example.
%
% For the feature development, the user pushes changes to the user's repository.
Feature development happens in the user's repository.
When the feature is implemented together with its tests, the user opens a merge request~(MR), i.e., a request to integrate their changes into the main branch.
% The merge request is submitted by the researcher that is responsible for the development from her/his repository into the central repository.
This triggers the CI pipeline, where the build system, CMake in the example, is used to check the compilation of the software on different platforms.
Once the software passes this stage of so-called build tests, the actual tests are executed on the GitLab runner.
Besides small-scale unit tests, this involves the execution of parameter studies and populates the respective folder structure with secondary data, as shown in~\cref{fig:testvis}.

The automatic execution of tests as part of the CI pipeline is an important aspect to maintained software quality, and simplifies re-integration.
A merge request triggers the execution of the CI pipeline, and the MR should only be accepted if all tests have passed.
This ensures that the integration of all changes, i.e., feature branch and master branch, do not lead to errors in parts of the software.
% The automatic execution aspect of tests in the  Continuous Integration pipeline simplify the integration process.
% It is executed as soon as a merge request is submitted by a member of the research group.
% In this step, existing tests that relate to other parts of the code are also executed. 
% Requiring all tests to pass the merge request ensures that errors were not caused elsewhere while a new methodology was developed.

We explain an important additional detail of our CI pipeline, geared towards the needs in CSE.
Before the quantification of tests causes tests to either fail or pass, results are processed that show \emph{why} the tests failed / succeeded.
Often, the textual output of the test environment is not sufficient to diagnose test failure.
Especially in the context of many CSE disciplines, test results require visualization in the form of diagrams or $2$D/$3$D visualization to determine the cause of an error.
For this purpose, the proposed CI pipeline from \cref{fig:ci_cd} contains jobs that export the Jupyter notebooks as HTML. 
% and submit them as blog posts in another static pages (GitLab) repository. 
% \todo[inline]{@Dennis: is this still up-to-date? I think with the artifact browsing options of GitLab/GitHub it is not necessary to do blog posts...TM: correct, resoved.}
\tm{The result is the complete visualization of test results, uniquely identified with a commit.} 
% This makes it possible to view the blog post in a Web browser and very effectively discuss the results.

% Only after the tests have been visualized, they are actually evaluated in terms of \texttt{pass} / \texttt{fail} in the pipeline.
% The status \texttt{pass} / \texttt{fail} in this stage concerns the fulfillment of some conditions of numerical results, e.g., rate of convergence greater than $2.0$, errors are below $\epsilon_{max}$.
% Of course, if the simulation crashes before producing results that can be evaluated, the CI pipeline indicates a \texttt{fail}.
\todo[inline]{Proposed change by @Dennis: Besides unit tests, the test suite comprises parameter studies that involve short simulations for varying grid refinement and/or other parameter values. For simple test cases with analytical reference solutions, convergence rates upon grid refinement are determined and compared to the expected values. These convergence tests are performed for a wide range of choices of other model parameters to ensure that the implementation handles these parameters correctly. For more complex physics, for which no analytical solution can be derived, tailored test cases are used to check if physically meaningful results are obtained upon specific parameter variations. For instance, in the context of computational fluid dynamics, one can check that the magnitude of the velocity scales as expected with the density of the considered fluid. These relationships between target quantities and variations in model parameters are visualized in the test pipeline such that this information is readily available to the developers in case a failure (i.e.\ an unexpected relationship) is detected.\\
Finally, we strongly advocate the use of regression tests, in which the result produced by a short simulation in the test pipeline is compared against a result obtained by the software at an earlier stage. We recommend that for any physical process that is implemented, a small simulation promoting that process is added to the test suite together with a reference solution obtained at the point of writing the test. Upon test execution, the newly produced results are compared to the reference solutions using tolerances that are small enough to capture physically relevant deviations. While this does not guarantee physically correct solutions, it helps to detect changes in the behavior of the simulator upon any changes to the code. This means that in case a bug fix leads to failing regression tests, the reference solutions has to be updated accordingly. In order to facilitate regression testing, we have developed a Python package that allows for the detection of deviations in simulation results, supporting a variety of standard file formats (\href{https://gitlab.com/dglaeser/fieldcompare/-/tree/main/fieldcompare}{gitlab.com/dglaeser/fieldcompare}).

TODO: Actually use fieldcompare in the CI, we currently still use the old package, but I need to first implement the field filtering that we use in the CI into the new package.}

Provided all tests pass, the acceptance of the MR in \cref{fig:ci_cd} is decided by the responsible team member, who can also provide feedback on code quality.
A web interface to git, such as GitLab, simplifies the code-review process within the research group.

% An important aspect of CI for CSE are tests that reproduce \emph{production}-level runs.
% The VV tests we address 
\todo[inline]{The HPC tests were not addressed in detail, and we don't yet have the solution for HPC reproducibility. We should discuss this.}
% Many of such tests require HPC resources to be executed properly.
% Desirably, the HPC center provides a way to access HPC resources for such tests in a convenient way.
% This is not yet the case at our university.
% So, instead of using a centralized service to execute such production-level tests, each researcher installs the required so-called \emph{runner} to execute pipelines.
% Then, the runner can login to the HPC system, using the user's cresentials, and submit jobs to the HPC system, correctly accounting for compute resources.
% While being suboptimal, it allows us to carry out production-level tests.
% The GitLab CI pipeline, outlined in \cref{fig:ci_cd} relies on the so-called \textit{GitLab Runner} to execute the tests. 
% The Runner plays an important role for the PRODUCTION tests that require larger computational resources.
% The Runner can be set up so that it uses containers as the execution environment for the pipeline and not affect the system it is running in.
% This is especially interesting for PRODUCTION tests that run on an high-performance computing cluster.
% In this case, the \textit{Runner} can submit a job on the HPC cluster over \textit{SSH} and wait for the results of the test.
% This decentralizes testing, because the researchers can install GitLab runners on their local machines, in effect enabling the Runners to log in to the cluster with their SSH credentials.
% Being identified this way, the Runner of each individual user will consume the computational resources of this specific user. 
% Therefore, it is not necessary to configure centralized testing resources on the HPC cluster. 
% In order to test their software within the CI pipeline, the users simply request for more resources on the cluster within their HPC projects and use the existing infrastructure. 


%  The GitLab \textit{Runner} furthermore generalizes the exexution environment as an \textit{Executor}, making it possible to use Singularity containers to encapsulate the software environment safely \citep{Singularity}.


==> sections/cross-linking.tex <==
\subsection{Cross-linking publications, software, and datasets} 
\label{ssec:cross-linking}

\todo[inline]{PASC review: - Findability: also for researchers who are not yet aware of these data}

\todo[inline]{PASC review: - PIDs for Code: Github/Zenodo or GitLab/Zenodo integratioon seem worthwile to men on}

\todo[inline]{PASC review: I am not convinced that "submission" is the optimal timepoint to integrate feature branches into the main branch. This should be done before submission.}


\todo[inline]{PASC review: extend the publication from arXiv to peer-review and demonstrate this with examples.}

\todo[inline]{PASC review: cover the publication process better and cover the scientific workflow - basically we did this by including secondary data into the publication. Although the publication is not a digital artefact generated by scientific software, results of the publication are, without them, there is no publication.}


\todo[inline]{PASC review: Highlighting differences between software and data repositories.}

This section covers one of the most important aspects of our proposed workflow: the cross-linking of the publication, the software and the data sets, i.e., connecting all digital assets of a particular publication.
We motivate this step from multiple perspectives.

First, the authors of the publication and their respective research groups need easy ways to retrieve all assets for a given publication, e.g., to continue their work.
This may happen at a significantly later point than the publication date, for example, when a previous idea is investigated further, or new funding is obtained.
Since research team members at universities are usually Ph.D. students and postdocs that leave the group every 1-5 years, cross-linking digital assets of a publication is crucial for sustainability.

Second, researchers who want to compare their own work to published results, need an easy way to determine all parameters used to obtain the results.
Scientific publications in CSE generally do not contain all metadata required to reproduce the results. 
Often, only the parameters relevant to the parameter variation are published, for instance, different fluid densities and viscosities, or parameters of numerical schemes investigated in the publication. 
All other parameters used by the research software that are not part of the parameter variation are not mentioned. 
However, these unmentioned parameters may be completely different in another CSE research software. 
Concretely, a publication may contain the parameters and information about approximating curvature for multiphase flow simulations, and no information about the solution of the multiphase pressure equation, since it is not related to the paper's topic. 
Reproducing the effect of the curvature model in another software on the numerical stability of the simulation, however, does require the metadata about the pressure equation and its discretization.
Therefore, archiving and cross-linking input data (input metadata) with a publication significantly increases reproducibility. 

Third, funding agencies are starting to require research to be Findable, Accessible, Interoperable, and Reproducible \citep{FAIR} for a certain number of years.
Hence, being able to retrieve snapshots and container images of software versions, experiment / simulation configurations, the input and result data sets, follows the FAIR principles closely~\citep{FAIR}.
This approach is especially applicable in CSE, where, compared to experiments, every step in the data processing pipeline is digital.
%Cross-linking of all digital assets following the FAIR~\citep{FAIR} principles, is the final step in our minimal workflow.

\begin{figure}[tb]
    \centering
    \includegraphics[width=0.6\linewidth]{images/cross-linking.pdf}
    \caption{Cross-linked publication, data and source code using Persistent Identifiers.}
    \label{fig:cross}
\end{figure}

\paragraph{Effect of cross-linking on the publications}
%Scientific publications are an appropriate way to document and communicate methodologies from CSE due to their mathematical nature.
If a publication serves as documentation of a method implemented in scientific software, the two should be cross-linked.
Extending the cross-linking to also include the data reported in the publication in the form of diagrams and tables (\emph{secondary data}) is the logical next step - especially considering \dg{their typically small size}.
% Scientific publications are appropriate documentation methods for the methods implemented by the scientific codes in Computational Science and Engineering (CSE), simply because the CSE methods are mathematical and can therefore not be documented in the source code in a didactical, easily understandable way.
% If a scientific publication is a form of documentation of the method implemented in the scientific code, then cross-linking the publication, the scientific code, and the datasets reported in the publication is a logical next step.
Without archiving and cross-linking secondary data, other researchers still nowadays resort to scanning diagrams from publications, which is especially prone to error when logarithmic scales are used.
From the point of view of the research group: once the researcher responsible for the results, and the part of the source code used to generate them, \tm{leaves} the group, it quickly becomes impossible to associate the source code and the datasets used in the publication. \todo{@TM: results (, data,) and the part of source code...?}
Even if all digital assets are archived locally at the research institution the problem still persists: over the years, many publications, code versions, and datasets are generated, so the problem of findability (F in FAIR~\citep{FAIR}) grows with time, if it is not technically handled. 
From the point of view of an external researcher: the cross-linking makes it possible to retrieve all (configuration and result) data needed for a direct comparison of methods for the same simulation problem (R in FAIR~\citep{FAIR}).

\paragraph{Effect of cross-linking on the data}
The lack of cross-linking severely complicates data re-use.
To draw new conclusions or derive new results (models) from existing data, detailed information about the method that generated the data is necessary: information usually available in a scientific publication and simulation input metadata.
A new application may make it necessary to apply a method beyond the parameter set used to generate the existing data: in this case, knowing acceptable parameter ranges and finding the specific version of the research software is again necessary.

\paragraph{Effect of cross-linking on the software}
From the perspective of sustainable scientific software development and increasing scientific software quality, the issues are the same for the software, like those mentioned above for the publication and the datasets. 
For example, having only a specific version of the scientific software available, checking the results becomes problematic if the result datasets need to be re-computed.
\dg{This is especially difficult if} this involves extensive simulations that require considerable computational resources and know-how in preparing parameter variations, performing simulations, and post-processing results.
Scientific methods are improved sequentially: every research step improves on existing methodology. 
These improvements often change only some sub-algorithms of an existing method.
Thus, introduced differences are difficult to discern in the scientific code, since even relatively small research software contains many relatively complex sub-algorithms and, moreover, grows in time.
Knowing which method is implemented by the specific version of the software becomes relevant as soon as we aim to compare two methods.

%\paragraph{\Minwf{} cross-linking}
The \minwf{} cross-linking connects all digital assets related to a scientific publication, excluding full simulation results and software containers, and it is very straightforward to apply.
This is important, since an overly complex workflow cannot be easily adopted with limited resources in university research groups.
%, and not linking all digital assets would fall short of the FAIR principles.
A straightforward cross-linking of publications, scientific software, and result data can be achieved using Persistent Identifiers~(PIDs), as shown in \cref{fig:cross}.
%
% At the latest here, but I guess somewhat earlier, we should have a picture that shows the cyclic workflow.
% I'll sketch something manually, and add it for discussion if the picture is suitable, as this one probably takes some more time.
% (I'm not super familiar with Inkscape}
%
As outlined in~\cref{ssec:vcs}, the cross-linking using PIDs starts at the point in the development when a report is written, that is, a preprint to be submitted to a scientific
journal, a technical report or an internal report about a failed research idea.
In \cref{fig:workflow-timeline} we visualize a timeline of a project and at which points the different parts of the workflow are placed.
%This, of course, may be slightly different, depending on the respective research group.
For the remainder of the paper, we use the term \emph{submission} to refer to publishing a preprint, submitting to a peer-review process, or preparing an internal technical report.

\begin{figure}[t]
    \centering
    % trim: left lower right upper
    \includegraphics[clip=true,trim={0.8cm 1.8cm 0cm 17.5cm}, width=0.6\linewidth]{images/pdf/workflow-timeline}
    \caption{Schematic of a (software) project timeline and the proposed workflow steps. Software feature and experimentation is developed iteratively until the point of satisfying results. Then the publication about the method and its results is prepared and finalized. Thereafter, the next feature is approached.}
    \label{fig:workflow-timeline}
\end{figure}

% Process that cross-links source code (archive, git tag, git repo URL), preprint (publication, report) and secondary data)
\todo[inline]{@Dennis: I rewrote the remainder of this paragraph while keeping the old version as comment. Please double-check. }
% \todo[inline]{Tomislav: add new figure that contains source code archive on the data repository.}
% At the time of submission, the feature (research idea) branch is integrated into the main (development) branch, followed by creating a snapshot of the source code version in the form of a \emph{git tag}.
% If the idea did not work, cross-linking is performed for the feature branch. 
% The data generated from the simulation is uploaded to a data repository, as is an archive of the source code.
% %, e.g., TUdatalib\footnote{TUdatalib is the service provided at TU Darmstadt}~\citep{TUdatalib}, or a similar service.
% The data repository creates a persistent identifier~(PID) (e.g. a DOI) for every uploaded digital asset, making them uniquely identifiable.
%y
% We separate the scientific data into \emph{primary data} and \emph{secondary data}.
% Primary data are large: in the context of CSE they are full simulation results.
% Secondary data are small datasets that are visualized in the publication as diagrams or tables and are instrumental in interpreting the results of the method implemented in the scientific software and described by the publication.
% \emph{In the \minwf{}, only the secondary data are considered.}
At the time of submission, all feature and bugfix branches required for the research idea have been merged into the research idea branch (see~\cref{ssec:vcs}).
This branch now contains the state of the code with which the results that appear in the report are produced, and it is identified uniquely by its current commit id.
At this point, the data produced by running the code in this state are available and are used to write up the report.
After finishing the report, a snapshot of the code and the data are published into two different datasets of a data repository as \eg 
TUdatalib\footnote{TUdatalib is the data repository service provided at TU Darmstadt}~\citep{TUdatalib} or a similar service.
The data repository creates a persistent identifier~(PID) (e.g. a DOI) for every uploaded digital asset, which can now be mentioned in the report such that readers can find
the associated data and software. Now, the report itself can be published to a manuscript repository (e.g. ArXiv~\citep{ArXiv}), which further produces a PID for the publication.
If the report corresponds to a research idea that has failed, data repositories at universities usually make it possible to publish the report internally and still obtain a PID
for internal use. 

At this point there are PIDs for the code, data and the report, but so far only the report contains cross-links to the other assets. The next step is to mention the report in the
descriptions of the datasets for code and data, and place the PID of the report in the metadata. Afterwards, a commit and git tag are created in the code repository (see~\cref{ssec:vcs}),
which add the three PIDs that were obtained up to now to its documentation. Afterwards, this git tag can also be mentioned in the metadata of all three publications.
This makes it possible to retrieve a snapshot of the source code, but also to locate the version control repository and check out the tag, and continue researching.
Note that git tags are not PIDs and can be changed by the developers, so tags do not meet the requirements typically posed on long-term availability.
This three-way cross-linking \minwf{} is depicted in the first part of \cref{fig:workflow-timeline} and enables the convenient retrieval of all digital assets.
The resulting cross-linked assets are shown in \cref{fig:cross}.

One of the differences between the minimum and the full workflow cross-linking is the type of data that is published. To clarify: We separate the scientific data into
\emph{primary data} and \emph{secondary data}. Primary data are large: in the context of CSE they are full simulation results.
Secondary data are small datasets that are visualized in the publication as diagrams or tables and are instrumental in interpreting the results of the method implemented
in the scientific software and described by the publication. \emph{In the \minwf{}, only the secondary data are considered.}

To facilitate the processing of the published secondary data, scripts that produce the figures and tables shown in the publication may be added to the data publication.
In this context, Jupyter notebooks~\citep{Jupyter} have emerged as a convenient way of processing data and documenting data workflows.
In our workflow, the data generated through simulation is processed in Jupyter notebooks~\citep{Jupyter} (see \cref{ssec:tests}).
% In the minimum workflow, the Jupyter notebooks~\citep{Jupyter} are additionally exported in the HTML format, within the directory structure shown in \cref{fig:testvis}.
% The HTML export makes it possible to view the results without actively running a Jupyter instance, enabling quick inspection.

The small secondary data (e.g. CSV files in \cref{fig:testvis}) are archived together with the Jupyter notebooks and their HTML exports, the tabular information of the parameter study that connects case IDs with parameters, and the simulation input files.
In other words, the secondary data archive contains the complete directory structure from \cref{fig:testvis}, including all parameter studies reported in a publication, but without the large simulation results. 
The tabular information of the parameter study should be saved in a text format (YAML, JSON, CSV, or similar) that can be easily read by a computer program (I in FAIR~\citep{FAIR}), but also easily read by a researcher trying to find the ID of a simulation from a parameter study, that was simulated using a specific set of parameters. 
This archive makes it possible for a researcher to quickly find a CSV file (F in FAIR~\citep{FAIR}) that stores the data used to visualize a specific diagram in a publication.
The secondary data archive generally has a size below $1$GB and can easily be uploaded to and downloaded from the data repository.

It is important to note that although relatively small in size compared to full simulation results, the datasets that belong to secondary data contain all the information relevant for judging the quality of the scientific results, comparing different methods, or performing regression tests (ensuring all existing tests still pass when adding new features).

% DENNIS: I commented this because I added the content to a paragraph further up
% Both the git tag, and the PID of the source code archive are mentioned in the publication, together with a link to the active version control repository. 
% This makes it possible to retreive a snapshot of the source code, but also to locate the version control repository and check out the tag, and continue researching.
% Although git tags are not PIDs and may be changed, we are not suggesting a technical solution that prevents this.
% Instead, we are suggesting a best practice in using git tags to retreive relevant software snapshots from the live git repository. 
% If, for some reason, the git tag has been removed / modified, the source code archive published on the data repository contains the information about the remote repository.

% DENNIS: I commented this because I added the content to a paragraph further up
% Once the source code archive and secondary data are published on the data repository and mentioned inside a publication, the publication is submitted to a manuscript repository (e.g. arXiv), which further produces the PID of the publication.
% The description of the git tag is then updated with the PID of the secondary data archive and the publication's PID, and the metadata of the secondary data on the data repository are updated with the git tag of the research software, and the PID of the preprint on arXiv.
% If the idea has failed, and an internal technical report is generated, data repositories at Universities make it possible to publish the report internally and still obtain a PID for internal use. 
% This three-way cross-linking \minwf{} is depicted in the first part of \cref{fig:workflow-timeline} and enables the convenient retrieval of all digital assets.
% The resulting cross-linked assets are shown in \cref{fig:cross}.

At this point, the publication may enter the peer-review process that results in reviewer comments. 
The application of reviewers' comments and further research of the method lead to the repetition of the above described process. 
If the new feature is researched and works well, it is integrated into the research idea branch, a new git tag is generated (see~\cref{ssec:vcs}), the source code archive and the
secondary data are updated as new versions on the data repository, the pre-print is modified accordingly with new cross-links, a new version of the preprint is submitted to \eg
ArXiv, and the metadata on the data repository is updated. 


Although listing \tm{the cross-linking steps} here may make the workflow seem complicated, applying \tm{the steps actually} takes at most a couple of work hours, \tm{maximally a workday for an individual researcher}, \tm{and} even less in a team effort. 
Compared to the number of person-months (sometimes person-years) generally necessary to investigate a research idea, half of a workday used to follow the FAIR principles and
increase significantly the quality of \tm{research results}\todo{Not just software} is an excellent investment.




==> sections/full-workflow-crosslinking.tex <==



\subsection{Cross-linking publications, software, datasets, and software images}

While the \minwf{} cross-linking ensures the source code, the publication, and the secondary data are cross-linked, it can be extended further with primary data and containers (see \cref{ssec:containerization}). 
Publishing and cross-linking primary data enables readers of the publication to gain further insights into the results and draw new conclusions.
Adding software containers to the cross-linking workflow enables results of the scientific software to be reproduced more easily and across different computing platforms.
Here the additional steps are covered, \emph{cf.} \cref{fig:workflow-overview}, that are used to achieve these improvements.

% Primary data
% Primary data that contains the complete simulation results is only relevant in two cases: either for a more in-depth result analysis (e.g., isolating issues, understanding details) or for drawing new conclusions from existing data, e.g. deriving new models.
The primary data is archived in a slightly different way than the secondary data because of its size.
Each parameter study is stored separately to enable the researcher to only download a specific parameter study, which saves time and network bandwidth.
The directory structure, shown in \cref{fig:testvis} is used similar to archiving secondary data, the only difference being that each parameter study is stored in a separate archive. 
This makes it possible for the researchers to access subsets of results, for example, "STUDY A" or "STUDY B" in \cref{fig:testvis}, with respective Jupyter notebooks, their HTML exports, and the parameter study tabular information.
Datasets that are generated for subsets of the primary data are uploaded to a data repository and their PIDs are used for cross-linking as described for the \minwf{} above.

% Singularity
% To increase the reproducibility, the software, along with its dependencies and the data required to generate both primary and secondary data, is containerized.
Containers in this respect can be seen as single image files that contain everything necessary to execute user-specified commands.
These commands are defined when the container is created, and, since containers are immutable, will produce the same result when invoked.
In our workflow we use Singularity containers~\citep{Kurtzer2017}, as the technology is supported by our HPC center, and the images are single files that can easily be
uploaded to a data repository. It is important to publish the recipe for building the image alongside with the actual image, as this is an important documentation of the
requirements and dependencies of the published research software. \dg{A} problem \dg{with the} code publication of the \textit{minimum workflow is that it} only
contains the research software itself. However, that may depend on several other software packages, specific compiler versions, etc. This can make it difficult for interested
peers to get the software running on their system, \dg{even if these dependencies are explicitly stated.}
Moreover, the software may only run with specific versions of these dependencies
or possibly produces different results with other versions.
The recipe for building the image explicitly documents how the environment of the researcher who produced the results
published in the report can be instantiated and the image enables users to directly spin up a container with this environment without having to install anything.
\dg{In order for this recipe to yield the same results over time, it is important that it uses a version-pinned base image and only installs pinned versions of the
dependencies.}
\todo[inline]{@Dennis: cite paper "Johnny doesn't know how to build"?}


==> sections/geophase-short.tex <==
\subsection{geophase}
\label{subsec:ccs}

The geophase library \citep{geophase} implements geometrical algorithms and models for intersecting non-convex polyhedral volumes with non-planar faces in the \cppl{} programming language. 
Those algorithms are used in \citep{Maric2020ccs} for the positioning of a piecewise linear fluid interface in an unstructured geometrical Volume-of-Fluid method for simulating two-phase flows \citep{Maric2018,Maric2020rev}. 
The development of the Consecutive Cubic Spline (CCS) interface positioning algorithm \citep{Maric2020ccs} in the geophase library serves as a case study for the proposed workflow for increasing the quality of scientific software.

\subsubsection{\Minwf{}}

The git VCS is used for version control (\cref{ssec:vcs}) and the geophase library \citep{geophase} is actively developed on TUGitlab \citep{TUGitLab}. 
To simplify cross-platform installation and handling of dependencies the CMake~\citep{CMake} build system is used (\cref{ssec:build-system}). 
For the submission of the CCS algorithm \citep{Maric2020ccs}, the cross-linking of the preprint, the source code and the resulting data was done (\cref{ssec:cross-linking}).
Applying the proposed minimal workflow in the peer-review process increases the transparency, because the reviewers and the rest of the scientific community can access the preprint, the source code and the data.

\subsubsection{\Fuwf{}}

Issue tracking (\cref{ssec:issue}) is used to track the status of the project on GitLab using Kanban boards. The Continuous Integration (CI) is used for "geophase" as described in \cref{ssec:continuous-integration}. 
As shown in \cref{fig:ci_cd}, this also includes publishing Jupyter notebooks and secondary data as CI artifacts, available for download from the GitLab/Hub web interface. 
% as blog posts in a separate git repository for GitLab static pages. 

For geophase, the results from successful CI pipelines are also publicly available \citep{geophaseCI}.
This makes it possible to quickly isolate possible negative effects between different versions, before quantifying them and testing them inside the CI pipeline.
For the submission, a Singularity \citep{Kurtzer2017} container is created (\cref{ssec:containerization}) that contains both the geophase repository and its software enviornment. 
The Singularity container is configured in a way that enables execution of different tasks with a single command:
\begin{itemize}
\item the geophase library can be cloned
\item the source code of the geophase library can be built using the dependencies stored in the container, 
\item all tests can be executed and re-started, 
\item the jupyter notebook in the container can be served from within a container to visualize results.
\end{itemize}
Currently, the generation of the Singularity container (although straightforward) is still done manually, because the delivery of the container is reserved for a submission. 
Alternatively, the creation of the Singularity container can easily be included into the CI pipeline, which would, in turn, result in Continuous Delivery across different platforms. 
The geophase library was developed using TDD (\cref{ssec:tdd}), the tests have been implemented using the GoogleTest testing framework and categorized using CTest. 

A more complex future step extends the use of the Singularity container to run performance tests on the HPC cluster as a part of the CI pipeline. 
% The complexity is not in including this step in the GitLab CI pipeline, this is relatively straightforward, the remaining question is how to organize further work on the software, when production tests take many days to complete.
Once the production test execution on the HPC cluster is integrated in the workflow shown in \cref{fig:ci_cd}, the next step is to automate the publishing of the data sets using the API of the data repository.
It is important to note, however, that it is not necessary to automate every aspect of the workflow, because new features are developed very slowly in scientific software, and satisfactory results are obtained sometimes after many months or years of work.




==> sections/geophase.tex <==
\subsection{geophase}
\label{subsec:ccs}

The geophase library \citep{geophase} implements geometrical algorithms and models for intersecting non-convex polyhedral volumes with non-planar faces in the \cppl{} programming language. 
Those algorithms are used in \citep{Maric2020ccs} for the positioning of a piecewise linear fluid interface in an unstructured geometrical Volume-of-Fluid method for simulating two-phase flows \citep{Maric2018,Maric2020rev}. 
The development of the Consecutive Cubic Spline (CCS) interface positioning algorithm \citep{Maric2020ccs} in the geophase library serves as a case study for the proposed workflow for increasing the quality of scientific software.

\subsubsection{\Minwf{}}

The git VCS is used for version control (\cref{ssec:vcs}) and the geophase library \citep{geophase} is actively developed on TUGitlab \citep{TUGitLab}. 
To simplify cross-platform installation and handling of dependencies the CMake~\citep{CMake} build system is used (\cref{ssec:build-system}). 
For the submission of the CCS algorithm \citep{Maric2020ccs}, the cross-linking of the preprint, the source code and the resulting data was done (\cref{ssec:cross-linking}).
Applying the proposed minimal workflow in the peer-review process increases the transparency, because the reviewers and the rest of the scientific community can access the preprint, the source code and the data.

\subsubsection{\Fuwf{}}

Issue tracking (\cref{ssec:issue}) is used to track the status of the project on GitLab using Kanban boards. The Continuous Integration (CI) is used for "geophase" as described in \cref{ssec:continuous-integration}. 
As shown in \cref{fig:ci_cd}, this also includes publishing Jupyter notebooks and secondary data as CI artifacts, available for download from the GitLab/Hub web interface. 
% as blog posts in a separate git repository for GitLab static pages. 

For geophase, the results from successful CI pipelines are also publicly available \citep{geophaseCI}.
This makes it possible to quickly isolate possible negative effects between different versions, before quantifying them and testing them inside the CI pipeline.
For the submission, a Singularity \citep{Kurtzer2017} container is created (\cref{ssec:containerization}) that contains both the geophase repository and its software enviornment. 
The Singularity container is configured in a way that enables execution of different tasks with a single command:
\begin{enumi}
\item the geophase library can be cloned
\item the source code of the geophase library can be built using the dependencies stored in the container, 
\item all tests can be executed and re-started, 
\item the jupyter notebook in the container can be served from within a container to visualize results.
\end{enumi}
Currently, the generation of the Singularity container (although straightforward) is still done manually, because the delivery of the container is reserved for a submission. 
Alternatively, the creation of the Singularity container can easily be included into the CI pipeline, which would, in turn, result in Continuous Delivery across different platforms. 
The geophase library was developed using TDD (\cref{ssec:tdd}), the tests have been implemented using the GoogleTest testing framework and categorized using CTest. 

A more complex future step extends the use of the Singularity container to run performance tests on the HPC cluster as a part of the CI pipeline. 
% The complexity is not in including this step in the GitLab CI pipeline, this is relatively straightforward, the remaining question is how to organize further work on the software, when production tests take many days to complete.
Once the production test execution on the HPC cluster is integrated in the workflow shown in \cref{fig:ci_cd}, the next step is to automate the publishing of the data sets using the API of the data repository.
It is important to note, however, that it is not necessary to automate every aspect of the workflow, because new features are developed very slowly in scientific software, and satisfactory results are obtained sometimes after many months or years of work.




==> sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}

% With increasing complexity of software systems in Computational Science and Engineering~(CSE) -- modern simulation software packages contain multiple hundreds of thousands, if not millions, of lines of code -- the cost of maintenance has increased accordingly.
Research software \dg{engineering} - crucial in \textbf{Computational} Science and Engineering - continues to \dg{find little application in academia, potentially due to beliefs that the costs outweigh the benefits}~\citep{2020:heroux:psip}.
\dg{However,} efficient and long-term CSE research is impossible without sustainable research software development: without modularity and adequate test coverage, straightforward integration of different research ideas, and the ability to find and reproduce research results from publications, many CSE research projects stall.

Ensuring the sustainability of research software is often challenging even for a single researcher - often a Ph.D. student. Focusing only on \dg{an upcoming} scientific publication means focusing on the next set of computations, often wholly disregarding the impact of changes in the research software on the existing code base.
Adding new functionality while ensuring that complex existing CSE methods continue to work as they should is more complicated when multiple researchers work together on the same code base.
Sustainable research software, therefore, must allow the integration of contributions from different researchers and ensuring that previous contributions work as expected. 
The software industry has already established principles, workflows, and tools to cope with %software complexity, maintainability, and quality. 
\tm{sustainable software development}.
These principles and workflows are widespread in larger scientific projects; however, they find little to no application in many smaller projects, particularly at universities.
In research, everything revolves around scientific publications. 
There is a need to \textbf{F}ind research software and data related to a publication and \textbf{A}ccess it. 
Once results are found and accessed,  there is a need to \textbf{I}nteract with them easily - to draw new conclusions, perform a more detailed analysis, \tm{apply the method outside of the original application-range}.
Finally, to extend or improve methods, being able to \dg{\textbf{R}euse and/or} \textbf{R}eproduce results from specific milestones is necessary.
The requirements mentioned above are the basis of the \href{https://www.go-fair.org/fair-principles/}{FAIR} principles \citep{FAIR}.
For reproducing results, the specific software configuration and its environment (dependencies), complete input data, and a result evaluation workflow are necessary.
Moreover, structured management of \emph{primary data} (\eg simulation results) and \emph{secondary data} (\eg diagrams and tables) is also necessary.

% While we find a potential myriad of reasons for the situation, we are convinced that a structured approach to software development, and use in experimentation, is required.

% Challenges: 
% 1. having access to complete results, not just processed data,
% 2. being able to process these results (non-binary non-proprietary formats), 
% 3. being able to reproduce the results using the software,
% 4. diverging software versions
% 5. thorough verification and validation 
% While we find a potential myriad of reasons for the lack of application of the available tools and workflows, we are convinced that sustainable software development practices are required and possible for research software developed at university research groups.

% As outlined above, two main challenges exist that should be addressed:
% \begin{enumi}
% \item developing sustainable research software, and,
% \item accessing and reproducing results from a publication.
% \end{enumi}

% One of the most crucial aspects of result reproduction is the trustworthiness of scientific results, i.e., that a measurement or simulation method is thoroughly verified and validated.
Access to the software and its configuration used in a publication is crucial for result reproduction. 
Without access to the CSE software, and its primary and secondary data, the only way to assess whether a numerical method is working is to re-implement it.
Re-implementation of published CSE results is extremely difficult - \tm{CSE methods are generally complex}, and not all details are available in a scientific publication.
% The lack of research data (source code, secondary and primary data) linked to CSE scientific publications imposes 
\tm{The need to re-implement published work is slowing} down research in CSE and introducing equally significant financial losses in public research funding.

% Without having access to the software used to generate/process data in a publication, and the access to the primary data (simulation results) and secondary data (diagrams, tables) from the publication, the only way to really know if a numerical method is working is to re-implement it, which is in most case very challenging or impossible, as crucial details are often omitted in a publication.
% Another important aspect is the ability to reproduce the results from a scientific publication using the research software.
% This, however is only possible if it is clear which particular version of the software was used to generate the results, and how the software and its input were configured.

% Repetition from above.
% Given an accessible software, publication metadata should be enriched with information on the used software versions and configurations.
% These requirements have led to the development of the FAIR~\cite{FAIR} principles to improve the \textbf{F}indability, \textbf{A}ccessibility, \textbf{I}nteroperability, and \textbf{R}euse of digital assets.

As for the challenge of developing sustainable research software, we argue that a careful integration of new features, involving automatic verification and validation tests must be done, and can be done in a relatively straightforward way in \tm{the university research environment}.
Without integration, research software is often developed in diverging directions, and integrating features quickly becomes intractable.
Computational sciences pose an additional challenge: large-scale tests that require high-performance computing are often necessary for verification and validation of the research software. 
% I removed the end of this phrase "that are rarely found in industrial applications.". I think in many engineering-related industries, that use simulations, heavy HPC stuff is actually done?
This requires careful design of certain
parts of the workflow.

% \jp{we could add links to the RSE initiatives.}
% \jp{Do we know a citation of some containerization paper that makes this point?}
% \jp{we could also do some analysis (I guess manually) which conferences included artifact evaluation in which year, so we can show a trend of the reproducibility necessity}
% Note that the two challenges mentioned above can be answered separately from each other.
% It is possible to reproduce scientific results from a poorly designed unsustainable numerical code and it is possible to develop a well-designed code whose results are challenging to reproduce.


% \jp{We should make the target audience clear: some of the bits and pieces are not addressing the challenges of 8000000000 USD-funded ECP projects, but are more common in academic settings.}
In this paper, we propose a workflow that addresses these challenges mostly based on standard software development practices applied to research software in CSE.
The workflow is lightweight and is focused on small research teams or individual researchers at universities, because university researchers seldom have dedicated personnel and resources that support the development of sustainable research software. 
In addition, we show at which points the workflow can be extended.
%to enrich its application in computational sciences.
% In particular, we highlight the inclusion of high-performance computing resources for testing and Jupyter notebooks in combination with static web pages for result visualization.
% Our examples are drawn from a multi-year project in the field of computational fluid dynamics~(CFD) and scientific computing.

% The workflow that we describe in the following sections is focused on research software in the fields of Computational Fluid Dynamics (CFD) and Scientific Computing (SC), although the challenges present in these research areas are surely similar to other fields of Computational Engineering \& Science.

% \jp{We need to motivate what are some of the challenges. Also we should highlight approaches to address them. I was thinking about the Journal of Open Source Software as an example.}


% \jp{What about related work?}

% \jp{How can we evaluate the approach? Potentially to show that it helped.}

% Literature survey
%\todo[inline]{@JP, @Dennis: please double-check + correct.}
\begin{table*}[!hbt]
		\begin{tabular}{@{} *6l @{}}    \toprule
				\emph{Publication} & \emph{Branching model} & \emph{TDD} & \emph{Cross-linking} & \emph{CI}  & (Meta)data standardization \\\midrule
				 \citep{Jimenez2017}
					 & -  & -  & -  & - & 1  \\ 
				 \citep{Fehr2016} 
					 & -  & -  & -  & - & 2  \\ 
				 \citep{Wilson2014} 
					 & 1  & 2  & -  & - & -  \\ 
				 \citep{wilson_good_2017}
					 & -  & -  & 3 & 1 & 3  \\ 
				 \citep{stanisic_effective_2015}
					 & 1  & -  & - & 1 & -  \\ 
				 \citep{anzt_towards_2019}
					 & 1  & -  & - & 5 & -  \\ 
				 \citep{riesch_bertha_2020}
					 & 1  & -  & - & 1 & 4  \\ 
				 \citep{sampedro_continuous_2018}
					 & 1  & -  & -  & 4 & - \\
					 \bottomrule
				 \hline
		\end{tabular}
		\caption{A comparison of the proposed workflow with other workflows. Similarity is expressed subjectively using numbers 1 (not similar) to 5 (very similar), or '-' for an aspect that is not addressed.}
		\label{table:comparison}
\end{table*}

Increasing the quality of research software is gaining a lot of traction in the CSE community. 
Initiatives such as Better Scientific Software (BSSw) \cite{BSSw} and its German and British equivalents, the National Research Data Initiative (NFDI) \citep{NFDI} (with a community-driven knowledge-base \citep{NFDI4IngKBase}) and the Sustainable Software Initiative \citep{SSI}, support sustainable research software development by organizing workshops and providing best practices to the CSE community.
\tm{The "Turing Way" handbook \citep{TuringWay} is a community-driven excellent source of information on increasing the reproducibility of research results in data science.}

A discussion on best practices to increase the quality of scientific software can be found in \citep{Wilson2014}, which comprise quality aspects of the source code (\eg consistent naming and formatting), quality assurance measures (automated build and test pipelines), design principles (\eg "don't-repeat-yourself") and technical aspects such as the use of version control systems.
%In \citep{Wilson2014}, modularity, consistent naming, formatting, automating builds and tests, use of the version control system, and data representation are suggested as means to increase research software quality. 

In \cite{stanisic_effective_2015}, the issue of reproducibility is addressed by combining a "git" version control workflow that includes research data, and Org-mode for the Emacs text editor research documentation. The workflow is minimalistic, but it is tied to the Emacs editor.

A distinction between replicability, reproducibility and reusability of research software is described in \cite{Fehr2016}. According to the authors, replicability of a computational experiment requires sufficient documentation on how to set up and run the program, while the automation and testing of this procedure is only recommended. Reproducibility of the results requires additional information on hardware and software dependencies, while reusability further demands modular software and a licensing model. The workflow presented in this work places automation at its core, with the aim of increasing the reproducibility. 
% In \cite{Fehr2016}}, reproducing results is based on extensive source code documentation, and automated unit, integration and system tests. While source code documentation is crucial for sustainable research software development and faster research, reproducing tests should be automated. The necessity for automating tests is brought by possible mistakes or lack of information in the documentation, that are easily missed, since the documentation is passive - it is not evaluated / executed. Should a test lack sufficient or accurate information, it either fails catastrophically, or reproduces erroneous results.

Making software publicly accessible as early as possible, making it easily found, applying a license compatible with its dependencies and ensuring transparent contribution and communication channels become relevant when research software attracts collaboration partners and starts growing into an open-source project \cite{Jimenez2017}. Moreover, we argue that early public access represents a psychological motivational factor for university research groups - Ph.D. students that are mainly responsible for new feature development, in our experience, place more focus on code quality if they are working on a publicly accessible code.

Continuous Integration (CI) for research software on HPC systems was proposed in \citep{sampedro_continuous_2018}, using a dedicated Jenkins test server in combination with a Singularity \citep{Singularity} registry  to ensure reproducibility of research results. This approach is very promising, especially regarding the use of Singularity images that encapsulate the computing environment of the research software. Since then, web-based version control services such as GitHub and GitLab offer Continuous Integration - online automatic testing systems, that are easy to set up and make the dedicated Jenkins test server unnecessary. 

Good enough practices in scientific computing according to \citep{wilson_good_2017} focus on data management, software, collaboration and project organization. Regarding data management, they recommend the archiving of
raw data while making it easily understandable.
Their software recommendations focus on code quality in terms of comments, function naming, etc., while their collaboration recommendations may nowadays be replaced by issue tracking available on git hosting sites. Good enough is a crucial attribute for small university research groups: a workflow must be simple enough to be quickly adopted by a small team of Ph.D. students and postdocs. %Easily understandable data makes the research easier at the point where previous methods should be extended or re-used by a successor of their original author.

% Continous Benchmarking CB - alternatively, Continuous Verification and Validation (VV) - is an extension of Continuous Integration including comparisons of test results with existing results either from previous milestones, from other research software, from experiments, or analytical solutions.

Continuous Benchmarking (CB) is a useful method to make sure that the performance of a software does not deteriorate over time.
A CB workflow that includes version control, a modern build system, automatic testing framework, code reviews, benchmark tests on HPC systems, storage of performance data and their automatic visualization is presented in \citep{anzt_towards_2019}. They realized all the aforementioned steps by relying on available web-based technologies, apart from result visualization: the authors have developed their own web-based solution for this task.

For many research software projects, performance may be a secondary goal that comes after ensuring that physically meaningful results are being computed. To this end, Continuous Verification and Validation (VV) may be done by comparing test results against previous milestones, other research software, experiments or analytical solutions where available.

The importance of automatic visualization of results and their communication to team members is emphasized in \citep{Khuvis2019}. The authors use a custom workflow to manage continuous integration of research software using git hooks that trigger automatic tests and email as means of communication of test results.

%\todo[inline]{@JP: a few concrete sentences on these two articles.}
% \citep{2020:heroux:psip, 2019:katz:rse}.

Jupyter \citep{Jupyter} represents a powerful CSE environment for literate programming - interleaving documentation and executable code in Jupyter notebooks makes it possible to combine test documentation (problem description, method description) with data generation (simulations, experimental data processing) and visualization. In \citep{Beg2021}, Jupyter notebooks are combined with Binder \citep{Binder} - a web service for building custom computing environments that contain the software and all its dependencies. Focus is placed on using Jupyter Notebooks and literate programming to initialize and perform computational studies and visualize results. This workflow is relevant regarding reproducing results and interleaving computation and documentation.

A tabular summary of the comparison between our proposed workflow and those reported so far in the literature is given in \cref{table:comparison}.

Our minimalistic workflow applies all elements of the workflows mentioned above in a way that makes it easily adoptable by small university research groups in CSE and applicable also to legacy research software. 
We rely entirely on existing web services and open-source software for version control, automatic testing, computing environments, data management, and visualization. 
%The researchers are not expected to provide Application Programming Interfaces (APIs) to use the proposed simplistic workflow with their research software.
Another distinctive feature of our workflow is the focus on the scientific publication and the peer-review process as a source of milestones that mark the points in research that require the reproduction of results. In an ideal world, integration and testing are continuous, however, conditions for research software development at universities are far from ideal. Tying integration and testing to writing a scientific paper (submission, revisions, acceptance) significantly reduces the workload overhead of university researchers while still ensuring sustainable research software development. 

The paper is structured as follows: first, we outline an overview of the general workflow in \cref{sec:workflow}.
\dg{\Cref{sec:minimal-workflow,sec:full-workflow} outline a basic and full version of our workflow presenting their different aspects in detail, that is,
which challenge is addressed, which technology is applied, what are potential impediments, and how to overcome them}.
We \dg{describe a minimal working example in~\cref{sec:minimal-example}, while} two case studies are presented in \cref{sec:case-studies} that show the positive impact when following the suggested workflow.
% We provide examples from the project mentioned and highlight how the workflow improved the project progress in \cref{sec:evaluation}.
Finally, we draw conclusions in \cref{sec:conclusions} and outline further activities required.

==> sections/issue-tracking-short.tex <==
\subsection{Issue tracking}
\label{ssec:issue}

% \todo[inline]{PASC review: The sugges on to use JIRA to manage datasets etc. is interes ng. However, I would consider it feasible to be adopted by researchers if there are automatic ways to create the issue from the simulation environment. Such need for integra on should be mentioned.}

% PASTED FROM POSTER
% Project management with research data (JIRA, TUGitLab Kanban board)
% \begin{itemize}
% \item Issue-Tracking
% \begin{itemize}
%     \item Sustainability
%     \item Idea, feature, bug (training, individual support)
% \end{itemize}

% \item Free data model: Flexibility

% \item Intuitive search: Traceability in the project context
% \end{itemize}
% PASTED FROM POSTER

There are two important aspects of research software development at universities that can be improved significantly by issue tracking.

First, the research software developed at university research groups is mainly developed by personnel that has non-permanent positions and leave after $1-5$ years, e.g., Ph.D. students or Postdocs.
Often, virtually no overlap period is available: the person responsible for a research direction often leaves before the new person arrives.
In addition, (undergraduate) students work on projects on a short-term basis.
This high turnover rate at university research groups, combined with contributions from different research directions and experience levels, demands documentation of the project status. 
Without project status documentation, repeating the predecessor's steps, discovering unaddressed bugs again, and the inability to understand the reasoning behind decisions already made in the project when inheriting an existing project all lead to an enormous waste of time and resources. 

Second, once the software is published, the scientific community is likely to find bugs or alternative applications for the software.
Simplifying bug reports or feature requests from the outside world is crucial for increasing research software quality.
Hence, keeping track of the status of the research software is utterly important, to allow the transfer of knowledge about open issues and potential limitations.


An issue tracking system helps in communicating such aspects clearly to new project members and people generally interested in the software project.
Issue tracking systems are typically freely available on web-based git services~\citep{GitLab,GitHub,Bitbucket}, and allow to track the status of the project.
Issues such as bugs, ideas, research cooperations, and peer-review comments are modeled as cards. 
The issue cards can be extended with links to the source code and input data and attachments (e.g., images from simulations),  and they support the chat functionality - placing the discussion about an issue in the issue itself such that it is easily findable and understandable.

%\paragraph{\Minwf{} issue tracking}
Defects are reported as bug reports, and ideas are maintained as feature requests.
%Issue trackers allow discussions per issue, which makes the reasoning for adding a specific feature in a certain way traceable, and allows a better understanding retrospectively.
Moreover, ideas can be broken down into smaller sub-tasks, simplifying the onboarding process.

A straightforward way to present and update issues is the well-known Kanban approach \citep{Sugimori1977}.
It consists of a board where the issues are moved between three columns: \emph{To Do}, \emph{In Progress} and \emph{Done}.
The issues can be labelled, e.g., bug, improvement, or others, and they can be grouped into project milestones. 
If actively maintained, the straightforward Kanban issue tracking simplifies the transition of research personnel, as the status of the project, including its current milestones, can easily be understood on the visual Kanban board.
This lightweight issue tracking is already sufficient for research software developed within individual Ph.D. / PostDoc projects.
More advanced approaches for collaborative projects that involve many projects and researchers may require a dedicated issue tracking software and more complex issue tracking workflows.

% Should this section be addressing more the management level in a project hierarchy?
% Then, maybe, we should specifically mention that some of the tasks listed here, should be carried out by a designated PM

% \paragraph{\Fuwf{} issue tracking}
% The advanced features of an issue tracker used in the full-workflow are most interesting to management personnel.
% They simplify the process to keep track of progress and reporting of publications, time management of employees and general project progress.
% The possibility to perform time tracking of each issue, to introduce different issue types, and to extend information stored in each issue results in statistical information.
% This data can be analyzed to identify how fast issues are being resolved, or to search for specific data in the project.

% Especially in large projects with different subprojects and many collaborators, the efficient retrieval of information is important.
% Different platforms, e.g., Redmine~\citep{Redmine}, Youtrack~\citep{Youtrack} or Jira~\citep{JIRA} offer such possibilities.
% Jira specifically provides the \emph{Jira Query Language}~(JQL) to specify database-like queries within the issue tracker, as shown in \cref{fig:jiraissue}.
% In \cref{fig:jiraissue}, JIRA is used as an advanced issue tracker with custom issue types and custom issue-related data, resulting in a database that simplifies status tracking for scientific data and related publications in large and long-term collaborative projects.
% If JIRA is used like this, JQL makes it possible to filter out publications and datasets based on metadata, e.g. physical parameters, methods used, acceptance status, authors, and similar.
% Adding the issue tracker to the cross-linking, \emph{cf.}~\cref{ssec:cross-linking}, enables project management to quickly access all relevant data from the issue tracking system.
% %
% \begin{figure}[tb]
% \centering
% \def\svgwidth{0.95\columnwidth}
% \footnotesize
%     \input{images/jira-oriented-workflow.pdf_tex}
%     \caption{The full-workflow issue-tracking with full cross-linking of issues, data sets, and publications.}
%     \label{fig:jiraissue}
% \end{figure}
%
% Another advantage Jira provides is its query language.
% When dealing with large collaborative projects where many tasks and people cooperate there is the need to find information  from the project efficiently.
% \emph{Jira Query Language} (JQL) allows users to search in terms of tasks with respect to the name of the assignee, the status of the task, the date it was created or resolved, priority and many more combinations of all of the above.
% Advanced issue trackers such as JIRA make it possible to introduce new issue types and extend the information related to these issues with metadata from the simulations.
% This is very powerful, as it enables searches for e.g. all publications and datasets from a project where some physical parameter within a given range was used, as shown in \cref{fig:jiraissue}.
% In \cref{fig:jiraissue} above, a query is performed by a user trying to find publications and datasets that belong to a specific project, that were created between the years $2018-2019$ involving the capillary rise simulation and refering some PID.


==> sections/issue-tracking.tex <==
\subsection{Issue tracking}
\label{ssec:issue}

% \todo[inline]{PASC review: The sugges on to use JIRA to manage datasets etc. is interes ng. However, I would consider it feasible to be adopted by researchers if there are automatic ways to create the issue from the simulation environment. Such need for integra on should be mentioned.}

% PASTED FROM POSTER
% Project management with research data (JIRA, TUGitLab Kanban board)
% \begin{itemize}
% \item Issue-Tracking
% \begin{itemize}
%     \item Sustainability
%     \item Idea, feature, bug (training, individual support)
% \end{itemize}

% \item Free data model: Flexibility

% \item Intuitive search: Traceability in the project context
% \end{itemize}
% PASTED FROM POSTER

There are two important aspects of research software development at universities that can be improved significantly by issue tracking.

First, the research software developed at university research groups is mainly developed by personnel that has non-permanent positions and leave after $1-5$ years, e.g., Ph.D. students or Postdocs.
Often, virtually no overlap period is available: the person responsible for a research direction often leaves before the new person arrives.
In addition, (undergraduate) students work on projects on a short-term basis.
This high turnover rate at university research groups, combined with contributions from different research directions and experience levels, demands documentation of the project status. 
Without project status documentation, repeating the predecessor's steps, discovering unaddressed bugs again, and the inability to understand the reasoning behind decisions already made in the project when inheriting an existing project all lead to an enormous waste of time and resources. 

Second, once the software is published, the scientific community is likely to find bugs or alternative applications for the software.
Simplifying bug reports or feature requests from the outside world is crucial for increasing research software quality.
Hence, keeping track of the status of the research software is utterly important, to allow the transfer of knowledge about open issues and potential limitations.


An issue tracking system helps in communicating such aspects clearly to new project members and people generally interested in the software project.
Issue tracking systems are typically freely available on web-based git services~\citep{GitLab,GitHub,Bitbucket}, and allow to track the status of the project.
Issues such as bugs, ideas, research cooperations, and peer-review comments are modeled as cards. 
The issue cards can be extended with links to the source code and input data and attachments (e.g., images from simulations),  and they support the chat functionality - placing the discussion about an issue in the issue itself such that it is easily findable and understandable.

%\paragraph{\Minwf{} issue tracking}
Defects are reported as bug reports, and ideas are maintained as feature requests.
%Issue trackers allow discussions per issue, which makes the reasoning for adding a specific feature in a certain way traceable, and allows a better understanding retrospectively.
Moreover, ideas can be broken down into smaller sub-tasks, simplifying the onboarding process.

A straightforward way to present and update issues is the well-known Kanban approach \citep{Sugimori1977}.
It consists of a board where the issues are moved between three columns: \emph{To Do}, \emph{In Progress} and \emph{Done}.
The issues can be labelled, e.g., bug, improvement, or others, and they can be grouped into project milestones. 
If actively maintained, the straightforward Kanban issue tracking simplifies the transition of research personnel, as the status of the project, including its current milestones, can easily be understood on the visual Kanban board.
This lightweight issue tracking is already sufficient for research software developed within individual Ph.D. / PostDoc projects.
More advanced approaches for collaborative projects that involve many projects and researchers may require a dedicated issue tracking software and more complex issue tracking workflows.

% Should this section be addressing more the management level in a project hierarchy?
% Then, maybe, we should specifically mention that some of the tasks listed here, should be carried out by a designated PM

% \paragraph{\Fuwf{} issue tracking}
% The advanced features of an issue tracker used in the full-workflow are most interesting to management personnel.
% They simplify the process to keep track of progress and reporting of publications, time management of employees and general project progress.
% The possibility to perform time tracking of each issue, to introduce different issue types, and to extend information stored in each issue results in statistical information.
% This data can be analyzed to identify how fast issues are being resolved, or to search for specific data in the project.

% Especially in large projects with different subprojects and many collaborators, the efficient retrieval of information is important.
% Different platforms, e.g., Redmine~\citep{Redmine}, Youtrack~\citep{Youtrack} or Jira~\citep{JIRA} offer such possibilities.
% Jira specifically provides the \emph{Jira Query Language}~(JQL) to specify database-like queries within the issue tracker, as shown in \cref{fig:jiraissue}.
% In \cref{fig:jiraissue}, JIRA is used as an advanced issue tracker with custom issue types and custom issue-related data, resulting in a database that simplifies status tracking for scientific data and related publications in large and long-term collaborative projects.
% If JIRA is used like this, JQL makes it possible to filter out publications and datasets based on metadata, e.g. physical parameters, methods used, acceptance status, authors, and similar.
% Adding the issue tracker to the cross-linking, \emph{cf.}~\cref{ssec:cross-linking}, enables project management to quickly access all relevant data from the issue tracking system.
% %
% \begin{figure}[tb]
% \centering
% \def\svgwidth{0.95\columnwidth}
% \footnotesize
%     \input{images/jira-oriented-workflow.pdf_tex}
%     \caption{The full-workflow issue-tracking with full cross-linking of issues, data sets, and publications.}
%     \label{fig:jiraissue}
% \end{figure}
%
% Another advantage Jira provides is its query language.
% When dealing with large collaborative projects where many tasks and people cooperate there is the need to find information  from the project efficiently.
% \emph{Jira Query Language} (JQL) allows users to search in terms of tasks with respect to the name of the assignee, the status of the task, the date it was created or resolved, priority and many more combinations of all of the above.
% Advanced issue trackers such as JIRA make it possible to introduce new issue types and extend the information related to these issues with metadata from the simulations.
% This is very powerful, as it enables searches for e.g. all publications and datasets from a project where some physical parameter within a given range was used, as shown in \cref{fig:jiraissue}.
% In \cref{fig:jiraissue} above, a query is performed by a user trying to find publications and datasets that belong to a specific project, that were created between the years $2018-2019$ involving the capillary rise simulation and refering some PID.


==> sections/minimal-working-example.tex <==
\section{Minimal working example}
\label{sec:minimal-example}

We have prepared a Minimal Working Example (MWE) - a template CSE research project - that can serve as basis for adopting the proposed workflow. The workflow MWE contains a numerical C++ application implemented as a version-controlled open-source project \citep{MWErepo}, that generates a small data set, visualized by a Jupyter notebook, referenced in a minimal example of a scientific report (publication) \citep{ResearchReport}.
% A MWE of a scientific report cross-linkins the source code snapshot and the secondary data with itself.

The MWE research software is a simple C++ application that evaluates numerical derivatives of a polynomial using finite differences in a 1D interval. The finite differences are compared against exact values for a prescribed polynomial. The MWE research software is version-controlled (\cref{ssec:vcs}), and built using the CMake build system (\cref{ssec:build-system}). The example data sets, the repository snapshot, the active repository, and the minimal report are all cross-linked (\cref{ssec:cross-linking}).

The MWE is archived at the \href{https://tudatalib.ulb.tu-darmstadt.de/handle/tudatalib/3522}{\textcolor{blue}{TUdatalib data repository}}. The research data \citep{Data} and the snapshot of the research code \citep{CodeSnapshot} are archived, and cited in the example Research Report \citep{ResearchReport}, along with the URL of the "live" code repository. Once the research report \citep{ResearchReport} is uploaded to the repository, the \emph{metadata} of the other data items are updated, by adding 'dc.relation.isreferencedby' element, that denotes the data item is referenced by another item. This way the \href{https://tudatalib.ulb.tu-darmstadt.de/handle/tudatalib/3530?show=full}{\textcolor{blue}{full metadata record}} of a data item on the repository stores the cross-linking information, that can be updated as data-items evolve. For example, as the peer-review process progresses or new milestones are reached, new sub-versions of data items obtain new DOIs that denote sub-versions, eg. \url{https://doi.org/10.48328/tudatalib-921.2} for a new version of the Research Report. This makes it possible to continue updating the Report, Data, Code Snapshot with the feedback from the peer-review process or during the development of new and improved methods.

A minimal CI pipeline is configured for the GitLab \citep{GitLab} MWE source code repository \citep{MWErepo}, demonstrating the use of Jupyter notebooks for data processing and visualization. The research data linked with the report \citep{ResearchReport} is the artifact generated by the CI pipeline \citep{Data}. For realistic CSE tests, Jupyter notebooks contain detailed information about the test setup: geometry of the problem, initial and boundary conditions, model parameters.


==> sections/pira-short.tex <==
\subsection{PIRA}
\label{subsec:pira}

PIRA\footnote{PIRA: \url{https://github.com/tudasc/pira}.}\citep{2018:lehr:pira, 2019:lehr:piraII} is a performance profiler for \cl{}/\cppl{} applications.
It consists of different modules, implemented in different languages, that are maintained across multiple repositories, and various other external dependencies.
Hence, a particular version of PIRA consists of particular versions of various software projects.
When applied to a target application, the user specifies a configuration file that determines various parameters.
In particular, how the target program is executed and where to store profiling results.
This configuration file is, in its nature, similar to simulation parameters.

\subsubsection{\Minwf{}}
As suggested in the proposed workflow, the project uses the git VCS.
PIRA includes its different components as \emph{git submodules}, i.e., it tracks a specific version of theses modules.
The project is implemented in Python and some of its dependencies are implemented in \cl{}/\cppl{}.
The build system CMake\citep{CMake} was used from the start for all native code modules.
For its publications, the respective version of PIRA was tagged, which also includes the specific version of the submodules.
The configuration files are stored in a separate git repository, and a branch is created for each publication.
Cross-linking, as proposed in this paper, was not performed for the initial PIRA publications as it was still unclear which services to use.

\subsubsection{Additional workflow components in PIRA}
PIRA introduced a particular branching model later in the project.
The motivation for its introduction was twofold: the release of PIRA as open source software, and multiple students working on PIRA.
To simplify contributing, and guarantee a certain level of quality, the Gitflow~\citep{Gitflow} model was adopted.
The introduction of the Gitflow model helped with stabilizing the project's public repository significantly.

In addition to the introduction of the Gitflow model, the issue tracker and continuous integration were introduced to improve software quality further.
The issue tracker is used to report bugs and suggest new features or usability improvements.
Student assistants contribute by taking over responsibility for a certain issue.
Following the Gitflow model, they create a new feature branch, implement the feature, and re-integrate it using a merge request.
Since the adoption of the Gitflow branching model, the issue tracker and continuous integration, the public repository contained only one partly dysfunctional commit, i.e., a specific version in which some of the unit tests were failing.
The CI helps significantly with the development of features in the software.

A sometimes overlooked aspect of a working CI environment is that it serves greatly as a reference of what \emph{should} work.
Especially in a university setting, e.g., students on-boarding for a Bachelor or Master thesis, being able to point to a working configuration and environment of the software is beneficial.
The on-boarding of students, before the introduction of CI, consisted of multiple meetings to set up the environment and install required dependencies.
The introduction of CI mandated to improve this aspect.
Moreover, students start with the CI configuration, and only \emph{specific questions} of the setup are asked and resolved in personal (or virtual) meetings.

Lately, the containerization of PIRA, to simplify the CI environment, and gain first experiences with using PIRA in the cloud~\cite{2020:sokolowski:hycloud} was started and is being explored further.

==> sections/pira.tex <==
\subsection{PIRA}
\label{subsec:pira}

PIRA\footnote{PIRA: \url{https://github.com/tudasc/pira}.}\citep{2018:lehr:pira, 2019:lehr:piraII} is a performance profiler for \cl{}/\cppl{} applications.
It consists of different modules, implemented in different languages, that are maintained across multiple repositories, and various other external dependencies.
Hence, a particular version of PIRA consists of particular versions of various software projects.
When applied to a target application, the user specifies a configuration file that determines various parameters.
In particular, how the target program is executed and where to store profiling results.
This configuration file is, in its nature, similar to simulation parameters.

\subsubsection{\Minwf{}}
As suggested in the proposed workflow, the project uses the git VCS.
PIRA includes its different components as \emph{git submodules}, i.e., it tracks a specific version of theses modules.
The project is implemented in Python and some of its dependencies are implemented in \cl{}/\cppl{}.
The build system CMake\citep{CMake} was used from the start for all native code modules.
For its publications, the respective version of PIRA was tagged, which also includes the specific version of the submodules.
The configuration files are stored in a separate git repository, and a branch is created for each publication.
Cross-linking, as proposed in this paper, was not performed for the initial PIRA publications as it was still unclear which services to use.

\subsubsection{Additional workflow components in PIRA}
PIRA introduced a particular branching model later in the project.
The motivation for its introduction was twofold: the release of PIRA as open source software, and multiple students working on PIRA.
To simplify contributing, and guarantee a certain level of quality, the Gitflow~\citep{Gitflow} model was adopted.
The introduction of the Gitflow model helped with stabilizing the project's public repository significantly.

In addition to the introduction of the Gitflow model, the issue tracker and continuous integration were introduced to improve software quality further.
The issue tracker is used to report bugs and suggest new features or usability improvements.
Student assistants contribute by taking over responsibility for a certain issue.
Following the Gitflow model, they create a new feature branch, implement the feature, and re-integrate it using a merge request.
Since the adoption of the Gitflow branching model, the issue tracker and continuous integration, the public repository contained only one partly dysfunctional commit, i.e., a specific version in which some of the unit tests were failing.
The CI helps significantly with the development of features in the software.

A sometimes overlooked aspect of a working CI environment is that it serves greatly as a reference of what \emph{should} work.
Especially in a university setting, e.g., students on-boarding for a Bachelor or Master thesis, being able to point to a working configuration and environment of the software is beneficial.
The on-boarding of students, before the introduction of CI, consisted of multiple meetings to set up the environment and install required dependencies.
The introduction of CI mandated to improve this aspect.
Moreover, students start with the CI configuration, and only \emph{specific questions} of the setup are asked and resolved in personal (or virtual) meetings.

Lately, the containerization of PIRA, to simplify the CI environment, and gain first experiences with using PIRA in the cloud~\cite{2020:sokolowski:hycloud} was started and is being explored further.

==> sections/scientific-software-quality-workflow.tex <==
\section{A workflow for increasing the quality of scientific software}
\label{sec:workflow}


\todo[inline]{PASC review: consider reordering points to better introduce the reader to the workflow - a user story would help more.}

\todo[inline]{PASC review: figure 1 hard to interpret, see reviewer 3 response}

\todo[inline]{PASC review: unclear why sustainable software  and accessing and reproducing results need to be resolved.}

\todo[inline]{PASC: re-design of the workflow on HPC systems is not discussed in detail.}

\todo[inline]{PASC review: Integration alone with some testing is not sufficient for sustainable software: limited resources, university research groups, we are not saving the planet here.}

\todo[inline]{@Dennis: should we rename TDD to RQ-Driven-Development? Yes, not sure if I can do this before 06.08.}

%We propose the following workflow for increasing the quality of scientific software, outlined in detail in the following subsections.
An overview of our workflow's components is shown in \cref{fig:workflow-overview}.
The schematic highlights the aspects that we consider as the minimum workflow, while pointing out useful additions.
% However, as we explain in \cref{sec:case-studies}, not all additions are fundamental for all kinds of projects.
Projects should establish the minimum aspects first, and then increase towards the full workflow, as suggested in~\citep{2020:heroux:psip}.
This keeps initial investment manageable and introduces only minimal overhead to the general organization of the project.

\begin{figure}[tb]
    \centering
    % trim={<left> <lower> <right> <upper>}
    %\includegraphics[clip=true,trim={2.5cm 3.9cm 0.7cm 18.3cm},width=0.95\linewidth]{images/pdf/workflow-overview.pdf}
    \includegraphics[clip=true,trim={1.3cm 20.5cm 3cm 0.1cm},width=0.6\linewidth]{images/pdf/workflow-overview-v3.pdf}
    \caption{Overview of the proposed workflow and the technologies used. Elements in the lower white area show the \minwf{} steps. The elements along the gradient are recommended elements that comprise the \fuwf{}.}
    \label{fig:workflow-overview}
\end{figure}

At the very least, we recommend to
\begin{enumi}
\item use a \emph{version control system~(VCS)} for all source files of the software, as well as text files that hold experiment configurations,
\item use an established cross-platform \emph{build system} for the software artifacts, and,
\item perform \emph{cross linking} of the code, the scientific publications and data using the mechanisms provided by the VCS and persistent identifiers~(PID), e.g., digital object identifiers~(DOI).
\end{enumi}

Additionally, the project can include \emph{issue tracking} as an improvement, followed by \emph{continuous integration} and \emph{test-driven development} (TDD).
% In some contexts TDD may not be applicable, however, one should always aim for the benefits
% of using TDD, that is, high test coverage and the development of small, testable and loosely-coupled software units with a user-friendly API.
% (Dennis: I commented this because it appears already in the section on TDD)
As particularly beneficial we found using \emph{containerization} for both
testing purposes and for reproducible computational experiments.
Finally, the introduction of \emph{automatic quantification, visualization and evaluation on HPC systems} proved useful to early detect any degradation in performance or numerical quality.
The latter benefits significantly from a working continuous integration pipeline being available.
% Throughout the next sections, we present more details on the different aspects and the technologies we used. 

\dg{The workflow described in the remainder of this paper is built on top} of available and widely adopted open source software, and we \dg{refer} to the respective software documentation \dg{wherever appropriate}. The basic workflow is described first: \cref{ssec:vcs} covers version control systems, \cref{ssec:build-system} the use of the build system, and \cref{ssec:cross-linking} covers cross linking of publication artifacts.
Thereafter, additional components of the workflow are described: issue tracking~(\cref{ssec:issue}), continuous integration~(\cref{ssec:continuous-integration}), containerization~(\cref{ssec:containerization}), test-driven development~(\cref{ssec:tdd}), and automatic quantification and evaluation using HPC systems~(\cref{ssec:tests}).

%
% Simplified workflow part
\section{Minimal workflow}
\label{sec:minimal-workflow}

\input{sections/version-control}

\input{sections/build-system}

\input{sections/cross-linking}

%
% Additional stuff to increase value of workflow
\section{Full workflow}
\label{sec:full-workflow}

\input{sections/issue-tracking}

\input{sections/test-driven-development}

\input{sections/test-quantification-visualization}

\input{sections/containerization}

\input{sections/continuous-integration}

\input{sections/full-workflow-crosslinking}


==> sections/test-driven-development.tex <==
\subsection{Test-Driven Development for Research Software}
\label{ssec:tdd}

\begin{figure*}[tb]
    \centering
    \includegraphics[width=0.95\textwidth]{images/rse-tdd.pdf}
    \caption{Test-Driven Development (TDD) applied to research software in resource-limited university research setting. TDD is applied in a top-down approach, starting with the CSE application that should generate research results, then applying TDD to its sub-algorithms recursively, on a per-need basis.}
    \label{fig:rsetdd}
\end{figure*}

\todo[inline]{This section is meant to be a substitute for the two following sections
whose text I haven't deleted yet, it is just commented out in the .tex file. One thing I left out are the smoke and 
production tests - I thought they are not fundamental thing of TDD? We should
maybe discuss that.}


Test-Driven Development (TDD, \citep{Beck2003}) is a practice of writing test applications (programs) first, \tm{before implementing the algorithms that are supposed to deliver the test results.} 
This forces \tm{programmers} to think about the code from
the perspective of the user, which typically yields a cleaner API \tm{(Application
Programming Interface) - the kind of API, the programmers would like to use themselves.} 
%The TDD technique  tests exist for every piece of the code and it makes
%programmers develop small, unit-testable components.
% \todo[inline]{TM: Disagree: i can do TDD with huge monolithic functions, it will help define the API, but I can program large functions and not do unit tests.}

TDD consists of \tm{three phases}: red, green and refactor.
\tm{The first, \emph{red}, phase begins with the implementation of the test applications, and,
as no algorithmic implementation is available to perform the actual computation, the tests fail.}
The tests define the return types and arguments of algorithms used in the tests, thus defining the API of the algorithm library.
\tm{The algorithm implementation follows, and it is modified until the tests pass, to enter the \emph{green} phase of TDD.}
\tm{In the final, \emph{refactor} phase,} the passing tests now allow the developers to refactor the implementation while using the tests to verify that the algorithmic implementation still works as intended.
\tm{Refactoring is
done until a modular (re-usable and extensible) software design is achieved.}
Then, the next algorithm is approached, by starting over with writing the tests first.
% This iterative process and its stages is visualized in \cref{fig:schematic-tdd}.\todo{Lost figure?}

% In research software development, TDD may not always be easy to apply. 
% However,
% independent of the development process, we recommend to strive for the key benefits
% that TDD promises: high test coverage, small unit-testable components and a
% user-friendly API.

We propose an adaptation of the TDD approach to research software in CSE. Our top-down TDD for CSE research software is outlined in \cref{fig:rsetdd}. 
Numerical methods in CSE consist of different complex
sub-algorithms.
Some methods are based on rigorous mathematical theory and have provable properties, e.g., convergence, or error estimates, others are based on approximations whose errors cannot be theoretically estimated.
In both cases, extensive and automatic verification and validation are crucial, since proven properties are not equivalent to a correct implementation.
Moreover, if the implementation does not produce the expected results, it is necessary to determine which part of the method's implementation causes the
problem, which is generally done by testing.
\tm{If TDD is applied for the development of research software with the goal of producing the (test)} results for a scientific publication, \tm{the focus is shifted from attempting to implement low-level unit-tests of all algorithms, to preparing only those verification and validation tests, that are relevant for the subsequent scientific publication}.
\tm{This way, tests that are written first, without providing the algorithmic implementation, are very high-level CSE applications, for example: partial differential equation (PDE) solvers.
Existing publications, that are supposed to be outperformed, define the test results. 
Alternatively, the results are defined by experimental data, or by the method of manufactured solutions.
Without a single line of algorithmic implementation, it is therefore possible to define the type of primary data generated by the CSE high-level test application  (e.g., velocity, pressure, and temperature fields), and what is expected of them (macroscopic quantities, e.g. drag resistance), as shown in \cref{fig:rsetdd}. 
Furthermore, it is possible to visualize the not-yet-available (empty) results against expected results - on purpose generating an artificially failing comparison.}

\tm{Once the research tests are prepared, the algorithmic implementation follows for the high-level application, by re-using algorithms from legacy research software, or, if necessary, implementing algorithms from scratch.
For algorithms implemented from scratch, the RSE TDD approach branches off and cycles through its phases until the algorithms implemented from scratch are refactored, in a recursive top-down approach, since they also consist of sub-algorithms.
Re-used sub-algorithms from legacy code on every level are assumed to be working correctly, unless the TDD testing shows otherwise, in which case suspicious sub-algorithms are selected for further TDD, as shown in \cref{fig:rsetdd}.
When the high-level application is not generating correct results after completed algorithmic implementation, TDD is applied to its sub-algorithm that is selected to be the most likely cause of the problem during result visualization/analysis.
In CSE, algorithms are generally very complex because they model complex physical phenomena. 
For example, a PDE discretization that is unit-tested for a set of Initial and Boundary Value Problems (IBVP), does not necessarily work for a IBV problem outside of the tested set.
Automatic testing and visualization of results in the red phase help the programmers more easily isolate troublesome sub-algorithms that require more TDD.
This way, finalizing the green phase for the high-level application does not require unit-testing to be applied on every sub-algorithm of a CSE application, which is not possible to do in a university research setting because of the lack of dedicated resources. 
Only those sub-algorithms that are not correct in the context of expected research results are further developed with TDD.}
\tm{ As work continues on different scientific publications, the automatic test suite grows with new tests being added for new publications and the overall test coverage increases along the research roadmap, with working and useful sub-algorithms from both failing and succeeding research ideas integrated into the main software version following the RSE version-control branching model \cref{ssec:vcs}. 
}

% That is, a researcher may decide to program an application that addresses a specific
% research question first, and only afterwards implement the components required
% to make that application work. The difference is that this application is not a
% test, because typically the expected result of the application is not yet known.
% This technique may help the researcher to identify and implement only the components
% that are relevant for the research question.
%\todo[inline]{Disagree, let's talk, commented out above.}


% We propose to follow the principles of Test Driven Development (TDD)~\citep{Beck2003} to achieve, early on, a good foundation for test coverage and also to pay particular attention to code quality.

% \subsubsection{Test-Driven Development}
% TDD is a straightforward practice that significantly increases software quality and consists of two phases: red and green.
% It requires that tests -- typically unit tests -- are created \emph{before} the functionality, e.g., an algorithm, is implemented.
% This lets the developer focus on functional requirements and design aspects of the application programming interface~(API), as it is first perceived from a user's point of view.
% The result is, typically, a much cleaner and more thoroughly thought API~\citep{Mcconnell2004}.
% Next, all tests are executed, and, as no implementation is available, they fail -- the \emph{red} phase.
% % Edit Dennis: I commented out my \todo below as changing this would affect also
% % figure 6, etc.. Maybe too big of a change, and I am not sure what the common sense
% % on this is in the software industry. One could of course write "all" unit tests of
% % a software unit before implementing anything. Since the unit should be small,
% % this is probably still a valid approach (although I think the mainstream is 
% % the small incremental approach)
% % \todo[inline]{@Dennis: as far as I know from software engineering literature, they advocate that is important to go incremental in small steps. That is, write a single small unit test, it fails, write the associated code to make it pass, move on to the next test, etc. With a strong emphasis on never to write more code than necessary to make the test pass, and never work on more than one test at a time. The text here is written in plural, so suggesting that first ALL tests are written, and then implemented. I think this is not in line with the SE literature, maybe we should make that clear.}

% Thereafter, the algorithm is implemented and modified until the tests pass, to enter the \emph{green} phase of TDD.
% The test suite is extended with larger, so called \emph{smoke} tests, and completed with large, so called \emph{production} tests.
% Once the test suite is complete, the \emph{refactor} phase of TDD is entered.
% The developer revisits the code implemented and improves its readability, design and performance until satisfied.
% Then, the next algorithm is approached, by starting over with writing the tests first.
% This iterative process and its stages is visualized in \cref{fig:schematic-tdd}.

% \begin{figure}[tb]
%     \centering
%     % trim={<left> <lower> <right> <upper>}
%     \includegraphics[clip=true,trim={0.2cm 21.2cm 6.7cm 0.3cm},width=0.95\linewidth]{images/pdf/schematic-tdd.pdf}
%     \caption{Test-Driven Development: for each feature, first, tests are created. The functionality is implemented until the tests pass. Second, the code is refactored, i.e., improved until satisfactory. Third, the next feature is started.}
%     \label{fig:schematic-tdd}
% \end{figure}

% In particular when implementing complex algorithms, code quality is important, e.g., readability and performance.
% We recommend to follow easy principles that increase code quality.
% In addition, static checkers, e.g., clang-tidy\footnote{Clang Tidy, \url{https://clang.llvm.org/extra/clang-tidy/}, last access Dec. 2020.}, can help and evaluate the code to warn developers when problematic patterns are found.

% \subsubsection{Code Quality}

% \todo[inline]{PASC review: - "at this stage" not clear to me which stage you are referring to}

% % In theory this is no longer TDD...
% So called \textit{pseudocode programming}~(PP)~\citep{Mcconnell2004} can be used at this stage to improve productivity and code quality.
% In PP, the developer first outlines an algorithm's pseudocode as comments in the code.
% This is easier to write than actual code, hence, it helps the programmer formulate the algorithm quickly.
% Moreover, the much easier to understand pseudocode is left as comment, and documents the algorithm.
% Additional straightforward practices for increasing code quality \citep{Mcconnell2004} include:
% %
% \begin{itemize}
%     \item Naming entities, e.g., variables or functions, understandably.
%     \item Making functions difficult to use incorrectly and easy to use correctly~\citep{Meyers2005}:
%         \begin{itemize}
%             \item Reducing the number of arguments whenever possible.
%             \item Placing modified arguments either always first, or always last in the argument list.
%             \item Providing forwards for functions with commutative arguments.
%         \end{itemize}
%     \item Removing copies in the source code.
%     \item Ensuring functions and classes have a single responsibility.
%     % This Single Responsibility Principle (SRP) leads to modular and re-usable API.
% \end{itemize}
% %

% % Technical: testing framework
% \subsubsection{Test Infrastructure}
% Closely related to TDD is the choice of a suitable testing framework for the project.
% We argue that an \emph{established testing framework} should be used when writing tests.
% Testing frameworks provide advanced testing functionalities and simplify test creation significantly.
% They are well-tested and provide, e.g., advanced assertions that take floating point comparisons into account, which is crucial for scientific codes.
% In addition, typical features enable the filtering of specific tests at runtime, i.e., re-running only failing tests, or sharing code/data between tests through so-called \emph{test fixtures}.
% Finally, their advanced assertion mechanism simplifies additional output that makes it easier to understand why a test failed.
% % For example, tests implemented using a testing framework can be easily filtered during execution of the testing application.
% % Filtering tests makes it possible to easily re-run only the failed tests or run a specific category of tests.
% % Established testing frameworks provide mechanisms that simplify sharing data between tests, i.e., test fixtures.
% % This aspect of testing frameworks is crucial for scientific codes.
% % The assertions already available in testing frameworks also simplify additional output of data that is useful for understanding why a test has failed.

% % The RED TDD phase has two important aspects.

% % First, formulating the tests before the algorithms makes the programmer focus on the goals the algorithm should achieve.
% % For numerical methods, these goals are convergence, stability, accuracy with respect to exact solutions or experiments, etc. 
% % Formulating these goals concretely early on, in terms of tests that define and quantify errors, increases the quality of the scientific code.

% % The second aspect of the RED phase in TDD, programming the tests first makes the programmer formulate the interface for the algorithms - the application programming interface (API) - early on.
% % The API consits of the result that the algorithm should return, the arguments it takes, the name of the algorithm, does it belong in a hierarchy of algorithms or share data with other algorithms (is it object-oriented), etc.
% % Placing oneself into the role of a "user" of a not-yet programmed API motivates the programmer to write clean code \citep{Mcconnell2004} of the API of high quality : re-use data by encapsulation and inheritance, minimize the number of function arguments, prevent repetition, assign single responsibility to functions, etc.

% It is important to note that production tests for CSE applications typically require HPC systems, due to their complexity and demand for compute power.
% Hence, limiting the execution of such tests by guarding them with a well designed set of unit and smoke tests is crucial.
% Both should run fast to give the developer immediate feedback on fail or success of changes and only if chances are high that production tests will succeed they should be performed.

% This section covers aspects of test-driven development, code quality and software engineering's design principles only very briefly.
% We refer the interested reader to the cited literature.

% % With passing tests, algorithms programmed in a clean way and documented with pseudocode programming, we enter the GREEN phase of TDD.
% % At this stage, input data of the tests for the scientific code are small, so that the tests can be evaluated quickly during development.
% % These tests we call UNIT or SMOKE tests: they can be executed relatively quickly on a PC or a Workstation.
% % The UNIT tests are responsible for testing the smallest algorithmic units with the smallest inputs. 
% % For example, this could be tests that check if a polynomial interpolation is working, for testing root finders, or testing solutions of small linear systems.
% % The SMOKE tests check the full functionality of a complex numerical method, but with small input data: they are used to test production-level scientific codes with a very coarse input, that enables fast execution on a Workstation.
% % Once the UNIT and SMOKE tests are running, PRODUCTION tests are introduced.
% % For scientific software, PRODUCTION tests are often not additional tests, but simply SMOKE tests with the high input resolution that is used in production.
% % Execution of PRODUCTION tests requires the use of high-performance computing clusters. 
% % The automation of PRODUCTION tests is described in \cref{ssec:continuous-integration}.
% % A testing framework simplifies the test categorization significantly. 

% % Once the UNIT, SMOKE and PERFORMANCE tests are running, the next stage of TDD is the REFACTOR stage. In the REFACTOR stage, both the testing applications and the algorithmic API are checked again for code quality and refactored if necessary.

% % There is more to TDD \citep{Beck2003}, however, already incorporating the aspects described here increases software quality significantly.

==> sections/test-quantification-visualization.tex <==



\subsubsection{Test qantification and visualization}
\label{ssec:tests}

\begin{figure*}[tb]
    \centering
    \includegraphics[width=0.95\textwidth]{images/Cluster-Parameter-Study-Organization.png}
    \caption{Different parameter studies are orchestrated by a Study Runner. All studies are implemented using Jupyter notebooks, which contain a problem description and the visualization of results. This allows for \emph{live} inspection of test result data. Structured metadata is exported into files to be available for subsequent use in publications and data cross-linking.}
    \label{fig:testvis}
\end{figure*}

Testing scientific software involves running parameter variations, so-called studies, as shown in \cref{fig:testvis}.
They often include hundreds of simulations, so called cases, \emph{cf.}~\cref{fig:testvis}.
The large number of test cases makes it important to be able to quickly identify failing tests and re-run them after changing the algorithm implementation to fix the problem.
Hence, the respective data, input and output, needs to be well organized.
% on the HPC system.
% Here it is important to organize the results on the cluster, so that failing tests can be easily identified.

The main input of such parameter studies are simulation parameters that are varied across the components of a \emph{parameter vector}.
This is, typically, performed automatically by a \emph{study runner} on an available HPC machine, as the production tests consume a significant amount of resources to execute.
In addition to running the respective case, the study runner also builds a mapping, using unique IDs, from each simulation case to the particular input parameter vector used.
Moreover, it exports structured metadata \tm{stored in both human and machine-readable standardized and open file format}, that can be used subsequently as part of the cross-linking process, \emph{cf.} \cref{ssec:cross-linking}.
% It is, however, advisable to export all metadata into an SQL database, such that it can be explored using any SQL software.
\cref{fig:testvis} shows a possible organization of the data in folders with a naming scheme of simple ascending integers used as the unique IDs.
% The software used to generate the study is responsible for generating the simulation cases and providing a map, that maps a unique ID of a case in each study ($000,001,\dots$ in \cref{fig:testvis}) to a parameter vector from the space of parameters varied in the study.
% This kind of organization simultaneously helps find and re-run failed simulation tests on the HPC cluster and at the same time, structures the \emph{simulation metadata}.
% Structured metadata further simplifies re-use of the simulation data: if someone downloads our parameter variation from a data repository, this person can easily find sub-sets of results (secondary data in \cref{fig:testvis}, based on a criterion applied in the parameter study map. 
% The map can be stored differently and it is often specific to the scientific software.
% However, good practice is to additionally store this information into an SQL table: this makes the mapping between a simulation case or secondary data, and the parameter vector inter-operable because it can then be processed using any SQL database software.

Being able to examine test results of the parameter studies run as early as possible is crucial to catch problematic executions timely, i.e., stop their execution, thus, limit the \tm{wasting of compute resources, reduce the negative impact on the priority on the HPC machine, and speeding up the research process.} 
% Having available a "study runner" (cf. \cref{fig:testvis}) that varies the simulation input and runs parameter variations on the HPC cluster, being able to examine simulation results in real time is the crucial next step.
Being able to perform real-time analysis of test results is, thus, fundamental.
Manual inspection of tables and diagrams is \tm{a natural part of the research process: it is often not possible or necessary, and sometimes not tractable, to automatically quantify the comparison of secondary data, resulting in an automatic pass/fail status of the test.}
% If the real-time result analysis is not available, tests that are failing, but not critically failing, will continue to run and consume computing resources on the HPC cluster.
A straightforward solution to the challenge of (almost) real-time manual test result analysis is the use of Jupyter notebooks~\citep{Jupyter}. 
A Jupyter notebook is written for each individual study, \emph{cf.} \cref{fig:testvis}.
The project notebook, i.e., the one executing the study runner, is created to link all the other notebooks.
This effectively links together all the tests used to verify / validate the scientific software in a single place.

Each Jupyter notebook is used to document its parameter study.
\tm{The test documentation covers the mathematical description of the CSE problem that is solved by the test.}
Such descriptions include which equations are solved, the initial and the boundary conditions, as well as physical parameters that are investigated.
The Jupyter notebooks then process secondary data generated by the simulation (or a post-processing utility that runs alongside the simulation), and store them as ASCII CSV files in \cref{fig:testvis}.
The central project notebook can be viewed \emph{live} locally in a browser, after the Jupyter server is started remotely on the HPC cluster.
This straightforward use of Jupyter notebooks makes it possible to check simulation results of many studies / cases that may run for a long time on a cluster, and stop those early that are not generating satisfactory results.
\tm{Additionally, since Jupyter notebooks are used for sequential processing of secondary data they use as input, they are always executed anew, and do not require information on the sequence of execution of their cells (provenance).}

An important benefit of this visualization process is that diagrams and related secondary data processed by the notebooks are used directly in the scientific publication.
They are stored by the notebooks in dedicated folders, that can be easily synchronized with the publication folder, as soon as the results are satisfactory.
Moreover, the solution is well suited for \tm{cross-linking of digital research artifacts (cf. \cref{ssec:cross-linking}), containerization (cf. \cref{ssec:containerization}), and continous integration of research software (\cref{ssec:continuous-integration})}.

A Ph.D. or a postdoctoral researcher focusing on a CSE methodology will not generally have the resources needed to alter the file format of primary data from a legacy CSE research software, which is not the case for secondary data.

On the other hand, \emph{secondary data is precious}: It is the basis for acceptance or rejection of scientific publications, decisions on whether milestones have been reached, and conclusions about one method outperforming all others.
There are two challenges in handling secondary data that our workflow addresses: handling metadata and interoperability. 
We propose a very straightforward solution. 
Secondary data is minuscule compared to primary data. 
%counting approximately tens to hundreds of MB per publication. 
Storing secondary data using an ASCII CSV format while saving metadata alongside result data directly in the columns solves both the issue of handling metadata and the interoperability of secondary data.
However, storing metadata next to data in columns introduces information repetition. 
For example, one can think of secondary data as a vector (row) uniquely identified in a parameter variation by another vector - a vector of parameters. 
In parameter variations, other parameters are held constant as one parameter varies.
Established data formats (e.g., HDF5 \citep{HDF5}) rely on a tree structure to model parameter variations without repetition of values. 
Contrary to this approach, for secondary data, we repeat non-varying parameter values alongside varying parameter values and store both as secondary-data columns. 
This way, all secondary data, and metadata are stored in a single table in ASCII CSV. 
This approach makes our secondary data completely interoperable, as any software that can process tabular data can process our secondary data.
The information about which column stores metadata information and which secondary data becomes apparent if the column names follow the nomenclature from the scientific publication. 
Furthermore, this approach trivializes the inclusion of metadata into data analysis:  using metadata for sub-set selection and other statistical or sensitivity analyses. 
Not relying on complex file formats simplifies the processing of secondary data immensely and saves time, with a negligible overhead caused by (meta)data duplication.
A concrete example of storing metadata together with secondary data in tabular form is shown for hyperparameter tuning of an artificial neural network (NN) in \cref{table:metadata}. 
Fixing one parameter and varying others causes data duplication, which can be ignored for secondary data because of its small size, and potentially used in further data analysis to better understand, in this case, the training behavior of the NN model. 

\begin{table*}[!htb]
    \scriptsize
    \input{images/pinn-of-libtorch-table-example.tex}
    \caption{Storing metadata (hyperparameters) together with secondary data (epoch, MSE) in tabular form.}
    \label{table:metadata}
\end{table*}




==> sections/version-control.tex <==
\subsection{Version control branching-model for research software}
\label{ssec:vcs}

\begin{figure*}[htb]
    \centering
    % trim: left lower right upper
    \includegraphics[width=0.95\linewidth]{images/cse-rse-branching-model.xml.iodraw.pdf}
    \caption{Schematic of the relationship between the feature-based git branching model, the peer-review process, and the cross-linking of digital research artifacts (cf. \cref{ssec:cross-linking}).}
    \label{fig:branching}
\end{figure*}


% A known and widespread problem in scientific software developed at universities are the different versions created for different publications.
% These versions are commonly not (re-)integrated into a single coherent version of the particular software.
Without version-controlled software, research efforts are doomed to be repeated, which hinders progress and wastes funding resources.
% Especially at universities, where a lot of the effort is mustered by Ph.D. students and postdocs with limited-time contracts, the resulting challenges are manifold.
% One important challenge is the creation of an integrated version of the software.
Additionally, the transfer of the reasoning behind software design decisions is a challenge when the various versions diverge, and \tm{non-permanent research personnel} leaves the university.
The situation becomes particularly \dg{critical} whenever new Ph.D. students continue the work of a former Ph.D. student.
% The problem is not only in the final versions of the software, it is more granular.
% If the changes are commented properly, it is possible to recover the reasoning behind the changes, after the person that was working on the project is gone. 
% This is often necessary for scientific software developed at Universities, where Ph.D. students inherit codes from their predecessors, and struggle to decipher the motivation behind the changes.

The proposed workflow approaches the challenges \tm{posed by} (re-)in\-te\-gra\-tion \tm{of different research ideas} by adopting a branching model in a version control system that \tm{combines version control with research milestones and the scientific publication process, to finally cross-link source code, research reports and result data, thus ensuring all digital research artifacts related to a scientific publication or a research idea are easily found}.
A commonly used \tm{version control system} (VCS) is \emph{git}~\citep{Chacon2014}, and many available web interfaces, e.g., Gitlab~\citep{GitLab}, Github~\citep{GitHub}, or Bitbucket~\citep{Bitbucket}, simplify its use.
% Nevertheless, it is crucial to employ a so-called \emph{branching model}, e.g., Gitflow or Github-flow, to the use of git, to benefit most from its capabilities.
For successful \tm{integration of versions}, it is crucial to follow a so-called \emph{branching model}, e.g., Gitflow~\citep{Gitflow} or Github flow~\citep{Githubflow}, to benefit most from git's capabilities.
% The lack of integration of new changes as well as comments documenting their motivation are solved by properly using a Version Control System: a software that tracks changes in the project without duplicating files.
% The most widely used version control system is the "git" Version Control System (VCS) \citep{Chacon2014} with many available web interfaces that simplify its use, such as: GitLab \citep{GitLab}, GitHub \citep{GitHub} and Bitbucket \citep{Bitbucket}. 

% Here, we want to emphasize the importance of going beyond using "git". 
% Simply using "git" will not solve the problem of never merging different versions. 
% In order to solve this problem, a \emph{branching model} must be applied and rigorously upheld.

A branching model describes how an individual or a team manage different versions. 
\dg{With a focus on small university research teams, we suggest to use the simplest possible feature-based branching model while connecting it} \tm{with the scientific publication process} \dg{to simplify result reproduction,}\tm{schematically shown in \cref{fig:branching} for an example research project.}
A research idea \dg{may require a number of different new features, which are possibly developed in parallel and on different branches
by different members of the research institution}.
\tm{We do not show research-idea sub-features in \cref{fig:branching} for the sake of clarity.}
% A research idea generally leads to multiple new feature branches as well as branches \dg{for the development of common methodology}. 
We \dg{suggest to create} one new branch for each research idea that will contain everything \dg{that is} needed, from the perspective of the research software, for a scientific publication.
\dg{All newly developed features are merged into the research idea branch, and the research idea is finished once the results it delivers are of high
enough quality for a scientific publication, or, if the idea fails.}
\tm{The software quality - in terms of the quality of research output - is therefore connected to the quality assurance given by the peer-review process in our workflow.}
% A \textit{finished} research idea implemented in research software is therefore generates results of high-enough quality to write a pre-print and publish it on an open-access publication archive, e.g. arXiv \citep{arXiv}. 
\tm{Whether an idea worked or not}, it is beneficial to write up the work carried out in a report, explaining
future researchers what has been done, \dg{what worked and what did not}.
\tm{This way, the generally completely neglected, but extremely valuable, negative scientific results are documented, at least in internal, and much better, in publicly available reports.}
Another reason for an internal report would be when a researcher leaves the institution and there is unfinished
work that may be \tm{continued} by someone else.

\dg{Before writing up the report, any new developments in the main branch should be incorporated
into the research idea branch, and it should be verified that features that had been already present 
in the research software still deliver the same results. If not, it must be investigated if the
new behaviour is an improvement or} \tm{if errors were introduced.}
Ensuring that existing features deliver results of similar quality when integrating new features can be done manually; however, in CSE context this \dg{typically takes many person-hours, and thus}, using automatic testing and continuous integration (see~\cref{ssec:continuous-integration}) is much more efficient.

\dg{At this stage, the research idea branch is mature enough to produce the results for a report,
for instance, for submission to a scientific journal. We suggest to publish both the report
and the data discussed in it in order to receive persistent identifiers (PID) that can be used for
cross-linking (see~\cref{ssec:cross-linking}).
The software itself, in the state of the research idea branch that was used to produce the
published results, should now also be published on a data repository such as
\eg Zenodo \citep{Zenodo}, or TUDatalib \citep{TUdatalib} at TU Darmstadt. This yields another PID for the software.
Next, a new commit is created on the research idea branch, which contains
only changes to the \textit{readme} file of the repository, adding
to it the PIDs of the software, data and the report publications. This makes sure that any
published digital asset produced with the software is documented. Finally, this commit is
\textit{tagged}, following a naming convention established in the group.
For instance, \textit{tags} may contain the} \tm{abbreviation of the research idea}, \dg{the abbreviation of the
journal to which the preprint was submitted, and the state of the review process
(\eg submission, accepted, revision-1, revision-2, etc.). More details on this and the cross-linking
are discussed in~\cref{ssec:cross-linking}.
}

%\dg{As a side note, it should be mentioned that fixes for bugs on the development branch should \textit{not} be done on research idea branches. These should be addressed in separate bugfix
%branches that branch off the development branch directly and are incorporated as soon as the fix is finished. All research ideas that require this bug fix should then
%"cherry-pick" the bug fix or rebase on the development branch.}
% \todo[inline]{@DG/TM:It seems to me that bug fixes should be integrated into main/master and development. This might get clearer with a diagram}

% it should be integrated into the development branch of the project, using the provided \emph{merge request} functionality.
% Discussions within the merge request conserve otherwise implicit knowledge of implementation decisions, either as part of the discussion itself, or as added comments.
% Once integrated, feature/bugfix branches are deleted on the remote repository.
% The research idea branch is tagged with a so-called "git-tag" and an archive of the software is published on a data repository (e.g. Zenodo \citep{Zenodo}), to enable
% cross-linking (see~\cref{ssec:cross-linking}) with the report and the results.
% This ensures that there is an archived research software version with a Persistent Identifier (PID), generated by the data repository, that can be found and used to reproduce
% results from the report (issues with dependencies are mentioned in~\cref{ssec:cross-linking}). Besides this, we think that the git tag should be named according to a naming convention established in the research group, for instance, containing the 
% research subject and the abbreviation of the journal to which the preprint was submitted.

At this point, the research team may decide if they consider the results good enough for the research idea branch to be merged with the development branch.
\dg{If preexisting features have been further developed on the research idea branch, we strongly suggest to merge it such that future unrelated research ideas can 
benefit from these improvements.}
\dg{In either case, this branching model allows the next person to comprehend the developments on the research idea branch, and possibly, start developing a new research idea based
on the one described in the report.}

The feature branch model is used further in the same way during the peer-review process \dg{of a manuscript}. 
Review comments \dg{may} lead to new feature branches and \dg{bug fixes, which are all merged before producing new results.}
Once the new version of the manuscript becomes satisfactory, \dg{the process described above is repeated for this revision: 
an archive of the research software is uploaded as a new version of the existing data item on the data repository
and cross-linked with the publication as outlined in \cref{ssec:cross-linking},
and the branch is tagged again according to the tag naming convention, suffixed with the revision number and maybe information on relevant improvements.}
Once the publication is accepted, the research idea branch is merged into the main branch,
making sure that it contains all successful ideas from published peer-reviewed work.

We want to emphasize again that we recommend this workflow also for research ideas that failed, that is, publishing code, data and a report and link them to a specific tag
in the software repository. The team may decide to keep the code with the failed research idea as a separate branch or merge it into the development branch in order to
maintain these pieces of code, for instance, if it is likely that this work will be picked up again in near future.

% This makes it possible for the next person to create a version from the master branch, and benefit from all the enhancements the group has developed up to that point.

% As an important step in the proposed workflow, we suggest to index the software state every time a feature is integrated with a persistent identifier~(PID) in the form of a \emph{git tag}.
% Every time a feature is integrated, it should be indexed with a Persistent Identifier (PID) in the form of  a "git tag". 
The major (tagged) milestones in this git branching model therefore revolve around scientific publications - digital artifacts that matter most in university research. 
Of course, this does not mean that more granular information is not available: the team can generate additional git tags for developments they deem relevant.
The core idea is to utilise git tags from major publication milestones to increase transparency and help to ensure reproducibility of results for these publications. 

Finally, here are some general recommendations for using a VCS that are and should be fundamental practice:
% First, \emph{delete branches} when they are no longer needed, to keep the project VCS as clean as possible.
\emph{Write telling messages} when you commit changes, such that your project partners understand what has changed and why it was introduced.
\emph{Prefer small changes} per commit instead of minimizing the number
of commits. Each commit should introduce a single coherent change, which also makes
it easier to enrich that change with a descriptive commit message.
\emph{Avoid putting multiple features into one merge request}. If a merge request
introduces one single feature, then it is easy to give it a descriptive name.
Moreover, if the feature is developed in small and well-named commits, the code
reviewing process is much facilitated, as both the intent of the merge request
as well as the steps required to make it work are obvious.
\emph{Make sure all tests pass on each commit}. This is especially important for 
code that needs to be compiled, since commits on which the code does not build impede
the usage of tools like \emph{git bisect}. In particular, \emph{make sure the tests
always pass on the development branch}. In order to achieve this, we recommend to rebase
branches before merging them into \emph{development}, making sure that all tests still pass. 
This makes sure that there have not been any changes on the
development branch that cause the new tests of the feature branch to fail after the merge.


% Although it is a bad practice to keep many versions active, because all those versions (\textit{branches}), creating new versions is very usefu finished research idea
% implemented in research software therefore generates results of
% high-enough quality to write a pre-print and publisl when one wants to experiment with new techniques without influencing the main project. 
% If the version is successful, it should be integrated in the master branch, otherwise it should be tagged and the respective branch deleted locally and on the remote repository, to keep the branch structure as clean as possible.

% When different users get (\textit{pull}) and send (\textit{push}) their changes with respect to the version control repository, it is not only important to comment the changes appropriately, but also to keep the changes granular. 
% In other words, committing changes that took weeks across dozens of file  in a single commit should be avoided, as this defeats the purpose of recovering different states of development and increases changes of conflicts during integration (merge conflicts). 

% After a new change is made, the author (\textit{committer}) creates a request (\textit{merge request}) on the git server (e.g. GitLab \citep{GitLab}). 
% The merge request is handled by the principal investigator or the project supervisor: she / he can review the proposed changes and provide feedback.

% This workflow is the standard practice in the software industry, and, if applied with discipline, it can increase significantly the quality of scientific software as well.

%Merging  also provides a way to resolve conflicts. Conflicts occur when for example two people edit the exact same file.

%Lastly, another concept close to CI is Continuous Delivery (CD) there is no application to be deployed in this case. Instead, a plain website hosted on GitLab (GitLab Pages) or any other server can be set up to automatically being deployed at the end of the pipeline. This website can contain diagrams or other numerical results and can also be in the form of a blog, where each commit will map into a new post.
